Sparsity comparison of polytopal finite element methods

In this work we compare crucial parameters for efficiency of different finite element methods for solving partial differential equations (PDEs) on polytopal meshes. We consider the Virtual Element Method (VEM) and different Discontinuous Galerkin (DG) methods, namely the Hybrid DG and Trefftz DG methods. The VEM is a conforming method, that can be seen as a generalization of the classic finite element method to arbitrary polytopal meshes. DG methods are non-conforming methods that offer high flexibility, but also come with high computational costs. Hybridization reduces these costs by introducing additional facet variables, onto which the computational costs can be transfered to. Trefftz DG methods achieve a similar reduction in complexity by selecting a special and smaller set of basis functions on each element. The association of computational costs to different geometrical entities (elements or facets) leads to differences in the performance of these methods on different grid types. This paper aims to compare the dependency of these approaches across different grid configurations.

==> tikzlibrary3dtools.code.tex <==
%
%
%
%
%
%
%
%
\ProvidesFileRCS{tikzlibrary3dtools.code.tex}
\usetikzlibrary{3d,decorations,fpu}%
\usepackage{calculator}%
\makeatletter%
\ifnum\month>10\relax
\typeout{Hibernation season has just started.}%
\fi
\ifnum\month<5\relax
\typeout{Hibernation season has not yet ended.}%
\fi
\ifnum\month=2\relax
\ifnum\day=2
\typeout{Yay! Groundhog Day!}%
\fi
\fi
\def\tikz@td@extractpgfversionaux#1.#2.#3|#4#5#6;{\def#4{#1}\def#5{#2}\def#6{#3}}%
\def\tikz@td@checkversion{%
\edef\pgfutil@tmp{\noexpand\tikz@td@extractpgfversionaux\pgfversion|\noexpand\pgfutil@tmpa\noexpand\pgfutil@tmpb\noexpand\pgfutil@tmpc;}%
\pgfutil@tmp%
\pgfmathtruncatemacro{\pgfutil@tmpe}{ifthenelse(10*\pgfutil@tmpa+\pgfutil@tmpb<31,0,1)}%
\ifnum\pgfutil@tmpe=0%
\message{You are using a too old version of pgf (\pgfversion). You need at least
version 3.1.1 to use the features of this library.}%
\fi
\edef\pgfutil@tmpd{\expandafter\@firstoftwo\pgfutil@tmpc\empty}%
\pgfmathtruncatemacro{\pgfutil@tmpe}{ifthenelse(100*\pgfutil@tmpa+10*\pgfutil@tmpb+\pgfutil@tmpc<313,0,1)}%
\ifnum\pgfutil@tmpe=0%
\message{Some routines of 3dtools may not work because they rely on the pushing
and popping techniques that were added in version 3.1.3 (but the current version
is \pgfversion).^^J}%
\fi
\pgfmathtruncatemacro{\pgfutil@tmpe}{ifthenelse(100*\pgfutil@tmpa+10*\pgfutil@tmpb+\pgfutil@tmpc<316,0,1)}%
\ifnum\pgfutil@tmpe=0%
\def\pgfutil@pushmacro##1{%
    \xdef\pgfutil@pushmacro@string{\string##1}%
    \ifcsname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\else
        %
        \csname newcount\expandafter\endcsname\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname
    \fi
    \global\advance\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname 1\relax
    \global\expandafter\let\csname\the\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\pgfutil@pushmacro@string\endcsname##1%
}
\message{pgfutil@pushmacro fixed because current pgf version \pgfversion\space is smaller than 3.1.6.^^J}%
\fi
}%
\tikz@td@checkversion%
%
%
%
%
%
%
%
%
%
%
\newcommand{\orthmat}[3]{%
\pgfmathparse{cos(#1)*cos(#2)}%
\xdef\tikz@td@matAA{\pgfmathresult}%
\pgfmathparse{sin(#1)*cos(#2)}%
\xdef\tikz@td@matAB{\pgfmathresult}%
\pgfmathparse{-sin(#2)}%
\xdef\tikz@td@matAC{\pgfmathresult}%
\pgfmathparse{cos(#1)*sin(#2)*sin(#3)-sin(#1)*cos(#3)}%
\xdef\tikz@td@matBA{\pgfmathresult}%
\pgfmathparse{sin(#1)*sin(#2)*sin(#3)+cos(#1)*cos(#3)}%
\xdef\tikz@td@matBB{\pgfmathresult}%
\pgfmathparse{cos(#2)*sin(#3)}%
\xdef\tikz@td@matBC{\pgfmathresult}%
\pgfmathparse{cos(#1)*sin(#2)*cos(#3)+sin(#1)*sin(#3) }%
\xdef\tikz@td@matCA{\pgfmathresult}%
\pgfmathparse{sin(#1)*sin(#2)*cos(#3)-cos(#1)*sin(#3)}%
\xdef\tikz@td@matCB{\pgfmathresult}%
\pgfmathparse{cos(#2)*cos(#3)}%
\xdef\tikz@td@matCC{\pgfmathresult}}%
\tikzset{3d/.cd,phi/.initial=0,psi/.initial=0,theta/.initial=0,
install view/.style={/utils/exec=\tikzset{3d/.cd,#1}%
\orthmat{\pgfkeysvalueof{/tikz/3d/phi}}{%
\pgfkeysvalueof{/tikz/3d/psi}}{\pgfkeysvalueof{/tikz/3d/theta}},%
/tikz/x={({\tikz@td@matAA*1cm},{\tikz@td@matBA*1cm})},%
/tikz/y={({\tikz@td@matAB*1cm},{\tikz@td@matBB*1cm})},%
/tikz/z={({\tikz@td@matAC*1cm},{\tikz@td@matBC*1cm})}}}%
\def\pgfmathparse@td@FPU#1{\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{#1}%
\pgfmathsmuggle\pgfmathresult\endgroup}%
\def\pgfmathsetmacro@td@FPU#1#2{\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathsetmacro#1{#2}%
\pgfmathsmuggle#1\endgroup}%
%
\xdef\tikz@td@type{0}%
\long\def\tikz@td@raw@coord(#1){\csname tikz@dcl@coord@#1\endcsname}%
\long\def\tikz@td@makesenseof@coord#1{%
\expanded{\noexpand\pgfutil@in@{(}{#1}}%
\ifpgfutil@in@%
\tikz@td@parse@coord#1%
\else
\tikz@td@parse@coord(#1)%
\fi
}%
\long\def\tikz@td@parse@coord(#1){%
\pgfutil@tempcnta=0%
\pgfutil@for\pgf@tmp:={#1}\do{\advance\pgfutil@tempcnta by1}%
\ifnum\pgfutil@tempcnta=1\relax
\edef\pgfutil@tmp{\csname tikz@dcl@coord@#1\endcsname}%
\fi
\ifcase\pgfutil@tempcnta
\or
\edef\pgfutil@tmp{\csname tikz@dcl@coord@#1\endcsname}%
\or
\edef\pgfutil@tmp{#1,0}%
\or
\edef\pgfutil@tmp{#1}%
\fi%
\pgfmathparse@td@FPU{xcomp3(\pgfutil@tmp)}%
\edef\pgf@X{\pgfmathresult pt}%
\pgfmathparse@td@FPU{ycomp3(\pgfutil@tmp)}%
\edef\pgf@Y{\pgfmathresult pt}%
\pgfmathparse@td@FPU{zcomp3(\pgfutil@tmp)}%
\edef\pgf@Z{\pgfmathresult pt}}%
\pgfmathdeclarefunction{TD}{1}{%
\begingroup%
\pgfmathtdparse{#1}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
%
\pgfmathdeclarefunction{xcomp3}{3}{%
\begingroup%
\pgfmathparse@td@FPU{#1}%
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{ycomp3}{3}{%
\begingroup%
\pgfmathparse@td@FPU{#2}%
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{zcomp3}{3}{%
\begingroup%
\pgfmathparse@td@FPU{#3}%
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{TDx}{1}{%
\begingroup%
\edef\mycoord{\tikz@td@raw@coord(#1)}%
\pgfmathparse@td@FPU{xcomp3\mycoord}%
\pgfmathsmuggle\pgfmathresult\endgroup}%
\pgfmathdeclarefunction{TDy}{1}{%
\begingroup%
\edef\mycoord{\tikz@td@raw@coord(#1)}%
\pgfmathparse@td@FPU{ycomp3\mycoord}%
\pgfmathsmuggle\pgfmathresult\endgroup}%
\pgfmathdeclarefunction{TDz}{1}{%
\begingroup%
\edef\mycoord{\tikz@td@raw@coord(#1)}%
\pgfmathparse@td@FPU{zcomp3\mycoord}%
\pgfmathsmuggle\pgfmathresult\endgroup}%
\pgfmathdeclarefunction{TDunit}{1}{%
\begingroup%
\pgfmathsetmacro{\pgfutil@tmpv}{TD("#1")}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpn}{min(1,sqrt(TD("(\pgfutil@tmpv)o(\pgfutil@tmpv)")))}%
\ifdim\pgfutil@tmpn pt<0.002pt\relax
\PackageWarning{3dtools}{Vector too short, cannot normalize it.}%
\let\pgfmathresult\pgfutil@tmpv%
\else
\pgfmathsetmacro@td@FPU{\pgfutil@tmpn}{1/sqrt(TD("(\pgfutil@tmpv)o(\pgfutil@tmpv)"))}%
\pgfmathparse{TD("\pgfutil@tmpn*(\pgfutil@tmpv)")}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup}%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\tikzset{3d/record physical components/.code={%
\tikzset{every coordinate node/.append style={3d/store components}}},
3d/store components/.code={%
\edef\pgf@Z{\relax}%
\edef\pgfutil@tmpz{\relax}%
\expandafter\tikz@td@parse@coord\tikz@scan@point@coordinate%
\pgfmathsetmacro\pgfutil@tmpx{\the\pgf@x/1cm}%
\pgfmathsetmacro\pgfutil@tmpy{\the\pgf@y/1cm}%
\ifx\pgf@Z\pgfutil@tmpz
\pgfmathsetmacro\pgfutil@tmpz{screendepth(\pgfutil@tmpx,\pgfutil@tmpy,0)}%
\else
\pgfmathsetmacro\pgfutil@tmpz{screendepth(\pgf@X,\pgf@Y,\pgf@Z)}%
\fi
\expandafter\xdef\csname tikz@td@physical@x@\tikz@fig@name\endcsname{\pgfutil@tmpx}%
\expandafter\xdef\csname tikz@td@physical@y@\tikz@fig@name\endcsname{\pgfutil@tmpy}%
\expandafter\xdef\csname tikz@td@physical@z@\tikz@fig@name\endcsname{\pgfutil@tmpz}%
}}
\pgfmathdeclarefunction{TDphysx}{1}{%
\begingroup%
\ifcsname tikz@td@physical@x@#1\endcsname
\expandafter\edef\expandafter\pgfmathresult\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\else
\PackageWarning{3dtools}{Physical x component of #1 not stored. Setting it to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDphysy}{1}{%
\begingroup%
\ifcsname tikz@td@physical@y@#1\endcsname
\expandafter\edef\expandafter\pgfmathresult\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\else
\PackageWarning{3dtools}{Physical y component of #1 not stored. Setting it to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDphysz}{1}{%
\begingroup%
\ifcsname tikz@td@physical@z@#1\endcsname
\expandafter\edef\expandafter\pgfmathresult\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\else
\PackageWarning{3dtools}{Physical y component of #1 not stored. Setting it to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDphys}{1}{%
\begingroup%
\pgfmathsetmacro{\pgfutil@tmpx}{TDphysx("#1")}%
\pgfmathsetmacro{\pgfutil@tmpy}{TDphysy("#1")}%
\pgfmathsetmacro{\pgfutil@tmpz}{TDphysz("#1")}%
\edef\pgfmathresult{\pgfutil@tmpx,\pgfutil@tmpy,\pgfutil@tmpz}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\tikzset{3d/.cd,local ex/.initial={localex},local ey/.initial={localey},
local ez/.initial={localez},dual ex/.initial={dualex},dual ey/.initial={dualey},
dual ez/.initial={dualez},install dual basis/.code={%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\pgfmathsetmacro{\pgfutil@tmpxx}{\pgf@xx/1cm}%
\pgfmathsetmacro{\pgfutil@tmpxy}{\pgf@xy/1cm}%
\pgfmathsetmacro{\pgfutil@tmpxz}{nscreenx}%
\pgfmathsetmacro{\pgfutil@tmpyx}{\pgf@yx/1cm}%
\pgfmathsetmacro{\pgfutil@tmpyy}{\pgf@yy/1cm}%
\pgfmathsetmacro{\pgfutil@tmpyz}{nscreeny}%
\pgfmathsetmacro{\pgfutil@tmpzx}{\pgf@zx/1cm}%
\pgfmathsetmacro{\pgfutil@tmpzy}{\pgf@zy/1cm}%
\pgfmathsetmacro{\pgfutil@tmpzz}{nscreenz}%
\path (\pgfutil@tmpxx,\pgfutil@tmpxy,\pgfutil@tmpxz) coordinate (\pgfkeysvalueof{/tikz/3d/dual ex})
	(\pgfutil@tmpyx,\pgfutil@tmpyy,\pgfutil@tmpyz) coordinate (\pgfkeysvalueof{/tikz/3d/dual ey})
	(\pgfutil@tmpzx,\pgfutil@tmpzy,\pgfutil@tmpzz) coordinate (\pgfkeysvalueof{/tikz/3d/dual ez});
\typeout{((\pgfutil@tmpxx,\pgfutil@tmpxy,\pgfutil@tmpxz),(\pgfutil@tmpyx,\pgfutil@tmpyy,\pgfutil@tmpyz),(\pgfutil@tmpzx,\pgfutil@tmpzy,\pgfutil@tmpzz))}%
}}
\pgfmathdeclarefunction{TDlocalx}{1}{%
\begingroup%
\ifcsname tikz@td@physical@x@#1\endcsname
\expandafter\edef\expandafter\pgfutil@tmpx\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpy\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpz\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\pgfmathparse@td@FPU{(\pgfutil@tmpx)*(\pgf@xx/1cm)+(\pgfutil@tmpy)*(\pgf@xy/1cm)+(\pgfutil@tmpz)*(nscreenx)}%
\else
\PackageWarning{3dtools}{Physical x component of #1 not stored. Setting result to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDlocaly}{1}{%
\begingroup%
\ifcsname tikz@td@physical@y@#1\endcsname
\expandafter\edef\expandafter\pgfutil@tmpx\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpy\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpz\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\pgfmathparse@td@FPU{(\pgfutil@tmpx)*(\pgf@yx/1cm)+(\pgfutil@tmpy)*(\pgf@yy/1cm)+(\pgfutil@tmpz)*(nscreeny)}%
\else
\PackageWarning{3dtools}{Physical y component of #1 not stored. Setting result to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDlocalz}{1}{%
\begingroup%
\ifcsname tikz@td@physical@z@#1\endcsname
\expandafter\edef\expandafter\pgfutil@tmpx\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpy\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpz\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\pgfmathparse@td@FPU{(\pgfutil@tmpx)*(\pgf@zx/1cm)+(\pgfutil@tmpy)*(\pgf@zy/1cm)+(\pgfutil@tmpz)*(nscreenz)}%
\else
\PackageWarning{3dtools}{Physical z component of #1 not stored. Setting result to 0.}%
\edef\pgfmathresult{0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{TDlocal}{1}{%
\begingroup%
\ifcsname tikz@td@physical@z@#1\endcsname
\expandafter\edef\expandafter\pgfutil@tmpx\expandafter{\csname tikz@td@physical@x@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpy\expandafter{\csname tikz@td@physical@y@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpz\expandafter{\csname tikz@td@physical@z@#1\endcsname}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpa}{(\pgfutil@tmpx)*(\pgf@xx/1cm)+(\pgfutil@tmpy)*(\pgf@xy/1cm)+(\pgfutil@tmpz)*(nscreenx)}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpb}{(\pgfutil@tmpx)*(\pgf@yx/1cm)+(\pgfutil@tmpy)*(\pgf@yy/1cm)+(\pgfutil@tmpz)*(nscreeny)}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpc}{(\pgfutil@tmpx)*(\pgf@zx/1cm)+(\pgfutil@tmpy)*(\pgf@zy/1cm)+(\pgfutil@tmpz)*(nscreenz)}%
\edef\pgfmathresult{\pgfutil@tmpa,\pgfutil@tmpb,\pgfutil@tmpc}%
\else
\PackageWarning{3dtools}{Physical z component of #1 not stored. Setting result to 0.}%
\edef\pgfmathresult{(0,0,0)}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
%
%
%
%
%
\def\tizk@td@spaux#1#2#3#4#5#6{(#1)*(#4)+(#2)*(#5)+(#3)*(#6)}%
\pgfmathdeclarefunction{scalarproduct}{2}{%
\begingroup%
\pgfmathparse@td@FPU{\tizk@td@spaux#1#2}%
\pgfmathsmuggle\pgfmathresult\endgroup} 
%
%
\def\vpauxx#1#2#3#4#5#6{(#2)*(#6)-(#3)*(#5)}%
\def\vpauxy#1#2#3#4#5#6{(#4)*(#3)-(#1)*(#6)}%
\def\vpauxz#1#2#3#4#5#6{(#1)*(#5)-(#2)*(#4)}%
%
\pgfmathdeclarefunction{vpx}{2}{%
\begingroup%
\pgfmathparse@td@FPU{\vpauxx#1#2}%
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{vpy}{2}{%
\begingroup%
\pgfmathparse@td@FPU{\vpauxy#1#2}%
\pgfmathsmuggle\pgfmathresult\endgroup} 
\pgfmathdeclarefunction{vpz}{2}{%
\begingroup%
\pgfmathparse@td@FPU{\vpauxz#1#2}%
\pgfmathsmuggle\pgfmathresult\endgroup} 
%
%
\pgfmathdeclarefunction{axisangles}{1}{%
\begingroup%
\pgfmathsetmacro{\pgfutil@tmpa}{sqrt(TD("#1o#1"))}%
\edef\pgfutil@tmpb{\tikz@td@raw@coord#1}%
\pgfmathsetmacro{\pgftemp@x}{xcomp3(\pgfutil@tmpb)/\pgfutil@tmpa}%
\pgfmathsetmacro{\pgftemp@y}{ycomp3(\pgfutil@tmpb)/\pgfutil@tmpa}%
\pgfmathsetmacro{\pgftemp@z}{zcomp3(\pgfutil@tmpb)/\pgfutil@tmpa}%
\pgfmathtruncatemacro{\itest}{ifthenelse(abs(\pgftemp@z)==1,0,1)}%
\ifnum\itest=0%
	\pgfmathtruncatemacro{\jtest}{sign(\pgftemp@x)}%
	\ifnum\jtest=1%
		\edef\pgfutil@tmpc{0,0}%
	\else
		\edef\pgfutil@tmpc{180,0}%
	\fi	
\else
    %
	\pgfmathsetmacro{\pgfutil@tmpb}{acos(\pgftemp@z)}%
    \pgfmathsetmacro{\pgfutil@tmpa}{acos(\pgftemp@x/sin(\pgfutil@tmpb))}%
    \pgfmathsetmacro{\ntest}{abs(cos(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@x)%
		+abs(sin(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@y)+abs(cos(\pgfutil@tmpb)-\pgftemp@z)}%
    \ifdim\ntest pt<0.1pt
      \edef\pgfutil@tmpc{\pgfutil@tmpa,\pgfutil@tmpb}%
    \fi
	%
	\pgfmathsetmacro{\pgfutil@tmpb}{acos(\pgftemp@z)}%
    \pgfmathsetmacro{\pgfutil@tmpa}{-acos(\pgftemp@x/sin(\pgfutil@tmpb))}%
    \pgfmathsetmacro{\ntest}{abs(cos(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@x)%
		+abs(sin(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@y)+abs(cos(\pgfutil@tmpb)-\pgftemp@z)}%
    \ifdim\ntest pt<0.1pt
      \edef\pgfutil@tmpc{\pgfutil@tmpa,\pgfutil@tmpb}%
    \fi
	%
	\pgfmathsetmacro{\pgfutil@tmpb}{-acos(\pgftemp@z)}%
    \pgfmathsetmacro{\pgfutil@tmpa}{acos(\pgftemp@x/sin(\pgfutil@tmpb))}%
    \pgfmathsetmacro{\ntest}{abs(cos(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@x)%
		+abs(sin(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@y)+abs(cos(\pgfutil@tmpb)-\pgftemp@z)}%
    \ifdim\ntest pt<0.1pt
      \edef\pgfutil@tmpc{\pgfutil@tmpa,\pgfutil@tmpb}%
    \fi
	%
	\pgfmathsetmacro{\pgfutil@tmpb}{-acos(\pgftemp@z)}%
    \pgfmathsetmacro{\pgfutil@tmpa}{-acos(\pgftemp@x/sin(\pgfutil@tmpb))}%
    \pgfmathsetmacro{\ntest}{abs(cos(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@x)%
		+abs(sin(\pgfutil@tmpa)*sin(\pgfutil@tmpb)-\pgftemp@y)+abs(cos(\pgfutil@tmpb)-\pgftemp@z)}%
    \ifdim\ntest pt<0.1pt
      \edef\pgfutil@tmpc{\pgfutil@tmpa,\pgfutil@tmpb}%
    \fi
	%
\fi
\edef\pgfmathresult{\pgfutil@tmpc}%
\pgfmathsmuggle\pgfmathresult\endgroup} 
%
\pgfmathdeclarefunction{screendepth}{3}{%
\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{%
((\the\pgf@yx/1cm)*(\the\pgf@zy/1cm)-(\the\pgf@yy/1cm)*(\the\pgf@zx/1cm))*(#1)+%
((\the\pgf@zx/1cm)*(\the\pgf@xy/1cm)-(\the\pgf@xx/1cm)*(\the\pgf@zy/1cm))*(#2)+%
((\the\pgf@xx/1cm)*(\the\pgf@yy/1cm)-(\the\pgf@yx/1cm)*(\the\pgf@xy/1cm))*(#3)}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
%
\pgfmathdeclarefunction*{nscreenx}{0}{%
\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{((\the\pgf@yx/1cm)*(\the\pgf@zy/1cm)-(\the\pgf@yy/1cm)*(\the\pgf@zx/1cm))}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction*{nscreeny}{0}{%
\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{((\the\pgf@zx/1cm)*(\the\pgf@xy/1cm)-(\the\pgf@xx/1cm)*(\the\pgf@zy/1cm))}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction*{nscreenz}{0}{%
\begingroup%
\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
\pgfmathparse{((\the\pgf@xx/1cm)*(\the\pgf@yy/1cm)-(\the\pgf@yx/1cm)*(\the\pgf@xy/1cm))}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
%
\pgfmathdeclarefunction{normalcandidate}{3}{%
\begingroup%
\pgfmathtruncatemacro{\icase}{(abs(#1)>0)+2*(abs(#2)>0)+4*(abs(#3)>0)}%
\ifcase\icase
\message{All three coordinates are zero. No normal can be computed.^^J}%
\edef\pgfmathresult{0,0,0}%
\or
\edef\pgfmathresult{0,1,0}%
\or
\edef\pgfmathresult{0,0,1}%
\or
\edef\pgfmathresult{0,0,1}%
\or
\edef\pgfmathresult{1,0,0}%
\or
\edef\pgfmathresult{0,1,0}%
\or
\edef\pgfmathresult{1,0,0}%
\or
\pgfmathsetmacro{\normalization}{(#1)*(#1)+(#2)*(#2)}%
\pgfmathsetmacro{\nx}{-1*(#2)/sqrt(\normalization)}%
\pgfmathsetmacro{\ny}{#1/sqrt(\normalization)}%
\edef\pgfmathresult{\nx,\ny,0}%
\fi
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction{randompermutation}{1}{%
\begingroup%
\c@pgf@counta=0%
\edef\pgfutil@tmpa{0}%
\loop
\advance\c@pgf@counta by1%
\edef\pgfutil@tmpa{\pgfutil@tmpa,\the\c@pgf@counta}%
\ifnum\c@pgf@counta<#1\relax
\repeat
\loop
\advance\c@pgf@counta by-1%
\pgfmathtruncatemacro{\pgfutil@tmpb}{1+rnd*\c@pgf@counta}%
\pgfmathtruncatemacro{\pgfutil@tmpc}{{\pgfutil@tmpa}[\pgfutil@tmpb]}%
\ifnum\c@pgf@counta=\numexpr#1-1\relax
\edef\pgfmathresult{\pgfutil@tmpc}%
\else
\edef\pgfmathresult{\pgfmathresult,\pgfutil@tmpc}%
\fi
\edef\pgfutil@tmpd{\pgfutil@tmpa}%
\edef\pgfutil@tmpa{0}%
\pgfutil@for\my@item:={\pgfutil@tmpd}\do{%
\unless\ifnum\pgfutil@tmpc=\my@item
\unless\ifnum\my@item=0\relax
\edef\pgfutil@tmpa{\pgfutil@tmpa,\my@item}%
\fi\fi}%
\ifnum\c@pgf@counta>0\relax
\repeat
\pgfmath@smuggleone\pgfmathresult%
\endgroup}
\pgfmathdeclarefunction{take}{2}{%
\begingroup%
\c@pgf@counta=0%
\pgfutil@for\my@item:={#1}\do{%
\advance\c@pgf@counta by1%
\ifnum\c@pgf@counta<#2\relax
\ifnum\c@pgf@counta=1\relax
\edef\pgfmathresult{\my@item}%
\else
\edef\pgfmathresult{\pgfmathresult,\my@item}%
\fi\fi}%
\pgfmath@smuggleone\pgfmathresult%
\endgroup}
%
%
%
\pgfmathdeclarefunction{barycenter}{1}{%
\begingroup%
\edef\pgfutil@tmpb{0}%
\tikzset{3d/tmp/.code={\edef\pgfutil@tmpb{\the\numexpr\pgfutil@tmpb+1}%
\ifnum\pgfutil@tmpb=1
 \edef\pgfutil@tmpc{##1}%
\else
 \edef\pgfutil@tmpc{\pgfutil@tmpc+##1}%
\fi},3d/tmp/.list={#1}}%
\pgfmathsetmacro{\pgfutil@tmpc}{TD("\pgfutil@tmpc")}%
\pgfmathsetmacro{\pgfutil@tmpa}{1/\pgfutil@tmpb}%
\pgfmathparse{TD("\pgfutil@tmpa*(\pgfutil@tmpc)")}%
\pgfmathsmuggle\pgfmathresult\endgroup}%
%
%
\pgfmathdeclarefunction*{pos}{2}{%
\begingroup%
\c@pgf@counta=1%
\pgfutil@for\my@item:={#2}\do{%
\ifdim\my@item pt<#1pt%
\advance\c@pgf@counta by1%
\fi}%
\edef\pgfmathresult{\the\c@pgf@counta}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}
\pgfmathdeclarefunction*{x2d}{1}{%
\begingroup%
\pgf@process{\pgfpointanchor{#1}{center}}%
\pgfmathparse{\pgf@x}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
\pgfmathdeclarefunction*{y2d}{1}{%
\begingroup%
\pgf@process{\pgfpointanchor{#1}{center}}%
\pgfmathparse{\pgf@y}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
%
\tikzset{convex hull of/.code={%
\edef\pgfutil@tmpl{#1}%
\edef\pgfutil@tmpp{}%
\c@pgf@counta1%
\pgfutil@for\pgfutil@tmpa:={\pgfutil@tmpl}\do{%
\ifnum\c@pgf@counta=1\relax
\pgfmathsetmacro{\pgfutil@tmpb}{x2d("\pgfutil@tmpa")}%
\edef\pgfutil@tmpd{\pgfutil@tmpa}%
\else
\pgfmathsetmacro{\pgfutil@tmpc}{x2d("\pgfutil@tmpa")}%
\ifdim\pgfutil@tmpc pt<\pgfutil@tmpb pt\relax
\edef\pgfutil@tmpb{\pgfutil@tmpc}%
\edef\pgfutil@tmpd{\pgfutil@tmpa}%
\fi
\fi
\advance\c@pgf@counta by1%
}
\edef\pgfutil@tmpp{(\pgfutil@tmpd)}%
\edef\pgfutil@tmpj{\pgfutil@tmpd}%
\edef\pgfutil@tmpe{90}%
\edef\pgfutil@tmpk{1}%
\loop
%
\edef\pgfutil@tmph{\noexpand\@removeelement{\pgfutil@tmpd}{\pgfutil@tmpl}{\noexpand\pgfutil@tmpl}}%
\pgfutil@tmph
%
\c@pgf@countb1%
\pgfutil@for\pgfutil@tmpa:={\pgfutil@tmpl}\do{%
\pgfmathsetmacro{\pgfutil@tmpf}{Mod(atan2(y2d("\pgfutil@tmpa")-y2d("\pgfutil@tmpd"),
x2d("\pgfutil@tmpa")-x2d("\pgfutil@tmpd"))+\pgfutil@tmpe,360)}%
%
\ifnum\c@pgf@countb=1\relax
\edef\pgfutil@tmpg{\pgfutil@tmpf}%
\edef\pgfutil@tmpi{\pgfutil@tmpa}%
\else
%
\ifdim\pgfutil@tmpf pt>\pgfutil@tmpg pt\relax
\edef\pgfutil@tmpg{\pgfutil@tmpf}%
\edef\pgfutil@tmpi{\pgfutil@tmpa}%
\fi
%
\fi
\advance\c@pgf@countb by1%
}
%
\ifx\pgfutil@tmpi\pgfutil@tmpj\relax
\c@pgf@counta=2\relax
\else
\edef\pgfutil@tmpd{\pgfutil@tmpi}%
\edef\pgfutil@tmpp{\pgfutil@tmpp--(\pgfutil@tmpd)}%
\pgfmathsetmacro{\pgfutil@tmpe}{180+\pgfutil@tmpe-\pgfutil@tmpf}%
%
\advance\c@pgf@counta by-1%
\fi
\ifnum\pgfutil@tmpk=1\relax
\edef\pgfutil@tmpl{\pgfutil@tmpl,\pgfutil@tmpj}%
\edef\pgfutil@tmpk{0}%
\fi
\ifnum\c@pgf@counta>2\relax
\repeat
\edef\pgfutil@tmpp{\pgfutil@tmpp--cycle}%
%
\tikzset{insert path=\pgfutil@tmpp}%
}}
%
\tikzset{generous outside path/.style={overlay,insert path={[reset cm]
			(-16383.99999pt,-16383.99999pt) |-
			(16383.99999pt,16383.99999pt)|- cycle}},
		 generous outside path'/.style={overlay,insert path={[reset cm]
			(-16383.99999pt,-16383.99999pt) -|
			(16383.99999pt,16383.99999pt)-| cycle}}}
%
\tikzset{even odd clip/.code={\pgfseteorule}}			
%
\tikzset{%
	save named path/.code={\tikz@addmode{\pgfsyssoftpath@getcurrentpath\pgfutil@tmpf
		\global\expandafter\let\csname tikz@td@named@path@#1\endcsname=\pgfutil@tmpf}},
	use named path/.code={%
		\expandafter\pgfsyssoftpath@setcurrentpath\expandafter{\csname tikz@td@named@path@#1\endcsname}}
}
%
\pgfkeys{%
  /tikz/on layer/.code={
    \pgfonlayer{#1}\begingroup
    \aftergroup\endpgfonlayer
    \aftergroup\endgroup
  },
  /tikz/node on layer/.code={
    \gdef\node@@on@layer{%
      \setbox\tikz@tempbox=\hbox\bgroup\pgfonlayer{#1}\unhbox\tikz@tempbox\endpgfonlayer\egroup}
    \aftergroup\node@on@layer
  },
  /tikz/end node on layer/.code={
    \endpgfonlayer\endgroup\endgroup
  }
}
%
\def\node@on@layer{\aftergroup\node@@on@layer}
%
%
\long\def\pgfmathtdparse#1{%
\begingroup%
%
%
%
%
%
%
\edef\pgf@Xa{0pt}%
\edef\pgf@Ya{0pt}%
\edef\pgf@Za{0pt}%
%
\tikz@td@cc@parse+#1%
}%
\def\tikz@td@cc@parse{%
\pgfutil@ifnextchar>{%
%
\tikz@td@cc@end%
} 
{\pgfutil@ifnextchar+{%
%
\tikz@td@cc@add%
}{%
\pgfutil@ifnextchar-{%
\tikz@td@cc@sub%
}{%
\pgfutil@ifnextchar x{%
\tikz@td@cc@vecprod%
}{%
\pgfutil@ifnextchar o{%
\tikz@td@cc@scalprod%
}{%
\pgfutil@ifnextchar[{%
%
\tikz@td@cc@pgfparse%
}{%
\tikz@td@cc@end%
}%
}%
}%
}%
}%
}%
}%
%
%
%
\def\tikz@td@cc@end{%
\ifcase\tikz@td@type%
\pgfmathsetmacro{\pgftemp@x}{\pgf@Xa}%
\pgfmathsetmacro{\pgftemp@y}{\pgf@Ya}%
\pgfmathsetmacro{\pgftemp@z}{\pgf@Za}%
\edef\pgfmathresult{\pgftemp@x,\pgftemp@y,\pgftemp@z}%
\or%
\pgfmathsetmacro{\myxa}{\pgf@Xa}%
\pgfmathsetmacro{\myya}{\pgf@Ya}%
\pgfmathsetmacro{\myza}{\pgf@Za}%
\pgfmathsetmacro{\myxb}{\pgf@Xb}%
\pgfmathsetmacro{\myyb}{\pgf@Yb}%
\pgfmathsetmacro{\myzb}{\pgf@Zb}%
\pgfmathsetmacro{\pgftemp@x}{\vpauxx{\myxb}{\myyb}{\myzb}{\myxa}{\myya}{\myza}}%
\pgfmathsetmacro{\pgftemp@y}{\vpauxy{\myxb}{\myyb}{\myzb}{\myxa}{\myya}{\myza}}%
\pgfmathsetmacro{\pgftemp@z}{\vpauxz{\myxb}{\myyb}{\myzb}{\myxa}{\myya}{\myza}}%
%
\edef\pgfmathresult{\pgftemp@x,\pgftemp@y,\pgftemp@z}%
\or%
\pgfmathsetmacro{\myxa}{\pgf@Xa}%
\pgfmathsetmacro{\myya}{\pgf@Ya}%
\pgfmathsetmacro{\myza}{\pgf@Za}%
\pgfmathsetmacro{\myxb}{\pgf@Xb}%
\pgfmathsetmacro{\myyb}{\pgf@Yb}%
\pgfmathsetmacro{\myzb}{\pgf@Zb}%
\pgfmathparse@td@FPU{\myxa*\myxb+\myya*\myyb+\myza*\myzb}%
%
\fi%
%
\xdef\tikz@td@type{0}%
\pgfmathsmuggle\pgfmathresult\endgroup}%
%
\def\tikz@td@cc@add+{%
\def\tikz@td@cc@factor{1}%
\tikz@td@cc@factororcoordinate%
}%
\def\tikz@td@cc@sub-{%
\def\tikz@td@cc@factor{-1}%
\tikz@td@cc@factororcoordinate%
}%
\def\tikz@td@cc@vecprod x{%
%
\xdef\tikz@td@type{1}%
\edef\pgf@Xb{\pgf@Xa}%
\edef\pgf@Yb{\pgf@Ya}%
\edef\pgf@Zb{\pgf@Za}%
\edef\pgf@Xa{0pt}%
\edef\pgf@Ya{0pt}%
\edef\pgf@Za{0pt}%
\def\tikz@td@cc@factor{1}%
\tikz@td@cc@factororcoordinate%
}%
\def\tikz@td@cc@scalprod o{%
%
\xdef\tikz@td@type{2}%
\edef\pgf@Xb{\pgf@Xa}%
\edef\pgf@Yb{\pgf@Ya}%
\edef\pgf@Zb{\pgf@Za}%
\edef\pgf@Xa{0pt}%
\edef\pgf@Ya{0pt}%
\edef\pgf@Za{0pt}%
\def\tikz@td@cc@factor{1}%
\tikz@td@cc@factororcoordinate%
}%
%
%
%
\def\tikz@td@cc@factororcoordinate{%
\pgfutil@ifnextchar({%
%
\tikz@td@cc@coordinate%
}{%
\pgfutil@ifnextchar[{%
%
\tikz@td@cc@pgfparse%
}{%
\tikz@td@cc@parse@factor%
}%
}%
}%
%
%
%
\def\tikz@td@cc@pgfparse[#1]{%
%
\pgfmathsetmacro{\tikz@td@cc@factor}{\tikz@td@cc@factor*(#1)}%
%
\tikz@td@cc@factororcoordinate%
}%
%
\def\tikz@td@cc@parse@factor#1*({%
%
\pgfmathparse@td@FPU{#1*\tikz@td@cc@factor}%
\let\tikz@td@cc@factor=\pgfmathresult%
\tikz@td@cc@coordinate(%
}%
\def\tikz@td@cc@coordinate(#1){%
\tikz@td@parse@coord(#1)%
\pgfmathsetmacro{\pgf@Xa}{\pgf@Xa+\tikz@td@cc@factor*\pgf@X}%
\pgfmathsetmacro{\pgf@Ya}{\pgf@Ya+\tikz@td@cc@factor*\pgf@Y}%
\pgfmathsetmacro{\pgf@Za}{\pgf@Za+\tikz@td@cc@factor*\pgf@Z}%
\tikz@td@cc@parse%
}%
\tikzset{declare function={torusx(\u,\v,\R,\r)=cos(\u)*(\R + \r*cos(\v)); 
torusy(\u,\v,\R,\r)=(\R + \r*cos(\v))*sin(\u);
torusz(\u,\v,\R,\r)=\r*sin(\v);
torusvcrit1(\u,\th)=atan(tan(\th)*sin(\u));%
torusvcrit2(\u,\th)=180+atan(tan(\th)*sin(\u));%
torusvtest(\u,\v,\az,\el)=sin(-vcrit1(\u-\az,\el)+\v);
torusdisc(\th,\R,\r)=((pow(\r,2)-pow(\R,2))*pow(cot(\th),2)+%
pow(\r,2)*(2+pow(tan(\th),2)))/pow(\R,2);%
torusumax(\th,\R,\r)=ifthenelse(torusdisc(\th,\R,\r)>0,asin(sqrt(abs(torusdisc(\th,\R,\r)))),0);
}}%
%
\tikzset{3d parse/.style={%
insert path={\pgfextra{\pgfmathtdparse{#1}}(\pgfmathresult)}},
3d coordinate/.style args={#1=#2}{%
%
insert path={\pgfextra{\pgfmathtdparse{#2}}(\pgfmathresult) coordinate #1}}}%
\newcommand\pgfmathprintvector[2][]{%
\begingroup
\pgfkeys{#1}%
\pgfutil@tempcnta0%
\pgfutil@for\pgf@tmp:={#2}\do{\advance\pgfutil@tempcnta by1}%
\pgfutil@tempcntb1%
\pgfutil@for\pgf@tmp:={#2}\do{\advance\pgfutil@tempcntb by1%
\ifnum\pgfutil@tempcntb<\pgfutil@tempcnta
\pgfmathparse{\pgf@tmp}%
\pgfmathprintnumber{\pgfmathresult},%
\else
\pgfmathparse{\pgf@tmp}%
\pgfmathprintnumber{\pgfmathresult}%
\fi}%
\endgroup
}%
%
%
\tikzset{3d/projection precomputations/.code n args={3}{%
\pgfmathsetmacro{\pgfutil@tmpa}{TD("#2-#3o#1-#3")/TD("#2-#3o#2-#3")}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("#3+\pgfutil@tmpa*#2-\pgfutil@tmpa*#3")}%
},3d/projection of/.style args={#1 on #2--#3}{%
3d/projection precomputations={#1}{#2}{#3},%
insert path={[3d parse={(\pgfutil@tmpb)}]}
}}
%
%
\tikzset{3d/.cd,
plane through/.code args={#1 and #2 and #3 named #4}{%
%
\pgfmathsetmacro{\pgfutil@tmpa}{TD("#2-#1x#3-#1")}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpa)o(\pgfutil@tmpa)")}%
\ifdim\pgfutil@tmpb pt<0.01pt\relax
\PackageWarning{3dtools}{The points #1 and #2 and #3 are either too close to each other or almost
on one line, so not suited to define a plane.}%
\else
\pgfmathsetmacro{\pgfutil@tmpc}{1/sqrt(\pgfutil@tmpb)}%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("\pgfutil@tmpc*(\pgfutil@tmpa)")}%
\pgfmathsetmacro{\pgfutil@tmpe}{TD("#1")}%
%
\expandafter\xdef\csname tikz@td@plane@normal@#4\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@plane@point@#4\endcsname{\pgfutil@tmpe}%
\expandafter\xdef\csname tikz@td@dim@#4\endcsname{2}%
\fi
},%
plane with normal/.code args={#1 through #2 named #3}{%
\pgfmathsetmacro{\pgfutil@tmpn}{sqrt(TD("#1o#1"))}%
\ifdim\pgfutil@tmpn pt<0.02pt\relax
\PackageWarning{3dtools}{Normal (\pgfutil@tmpn) is too short.}%
\else
\pgfmathsetmacro{\pgfutil@tmpn}{1/\pgfutil@tmpn}%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("\pgfutil@tmpn*#1")}%
\pgfmathsetmacro{\pgfutil@tmpe}{TD("#2")}%
\expandafter\xdef\csname tikz@td@plane@normal@#3\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@plane@point@#3\endcsname{\pgfutil@tmpe}%
\expandafter\xdef\csname tikz@td@dim@#3\endcsname{2}%
\fi
},%
line through/.code args={#1 and #2 named #3}{%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("#1")}%
\pgfmathsetmacro{\pgfutil@tmpe}{TD("#2")}%
\pgfmathsetmacro{\pgfutil@tmpf}{TD("#1-#2o#1-#2")}%
\ifdim\pgfutil@tmpf pt<0.001pt\relax
\PackageWarning{3dtools}{The points #1 and #2 are too close to each other. No line defined.}%
\else
\expandafter\xdef\csname tikz@td@line@A@#3\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@line@B@#3\endcsname{\pgfutil@tmpe}%
\expandafter\xdef\csname tikz@td@dim@#3\endcsname{1}%
\fi
},%
line with direction/.code args={#1 through #2 named #3}{%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("#2")}%
\pgfmathsetmacro{\pgfutil@tmpe}{TD("#1+#2")}%
\pgfmathsetmacro{\pgfutil@tmpf}{TD("#1o#1")}%
\ifdim\pgfutil@tmpf pt<0.001pt\relax
\PackageWarning{3dtools}{The points #1 and #2 are too close to each other. No line defined.}%
\else
\expandafter\xdef\csname tikz@td@line@A@#3\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@line@B@#3\endcsname{\pgfutil@tmpe}%
\expandafter\xdef\csname tikz@td@dim@#3\endcsname{1}%
\fi
},%
sphere with center/.code args={#1 and radius #2 named #3}{%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("#1")}%
\expandafter\xdef\csname tikz@td@sphere@C@#3\endcsname{\pgfutil@tmpd}%
\expandafter\xdef\csname tikz@td@sphere@r@#3\endcsname{#2}%
\expandafter\xdef\csname tikz@td@dim@#3\endcsname{3}%
},
project/.code args={#1 on #2}{%
\expandafter\edef\expandafter\pgfutil@tmpd{\csname tikz@td@dim@#2\endcsname}%
\ifcase\pgfutil@tmpd
\PackageWarning{3dtools}{It is not particularly meaningful to project a point on a point.}
\or%
\expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#2\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#2\endcsname}%
\pgfmathsetmacro{\pgfutil@tmpd}{TD("(\pgfutil@tmpa)-(\pgfutil@tmpb)o#1-(\pgfutil@tmpb)")/TD("(\pgfutil@tmpa)-(\pgfutil@tmpb)o(\pgfutil@tmpa)-(\pgfutil@tmpb)")}%
\pgfmathsetmacro{\pgfutil@tmpc}{TD("(\pgfutil@tmpb)+\pgfutil@tmpd*(\pgfutil@tmpa)-\pgfutil@tmpd*(\pgfutil@tmpb)")}%
%
\tikzset{insert path={(\pgfutil@tmpc)}}%
\or%
\expandafter\edef\expandafter\pgfutil@tmpn{\csname tikz@td@plane@normal@#2\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@plane@point@#2\endcsname}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpn)o(\pgfutil@tmpa)-#1")}%
\pgfmathsetmacro{\pgfutil@tmpc}{TD("#1+\pgfutil@tmpb*(\pgfutil@tmpn)")}%
%
\tikzset{insert path={(\pgfutil@tmpc)}}%
\fi
}}
%
%
\tikzset{3d/intersection of/.code args={#1 with #2}{%
\expandafter\edef\expandafter\pgfutil@tmpd{\csname tikz@td@dim@#1\endcsname}%
\expandafter\edef\expandafter\pgfutil@tmpe{\csname tikz@td@dim@#2\endcsname}%
\edef\pgfutil@tmpde{\pgfutil@tmpd\pgfutil@tmpe}%
\edef\pgfutil@tmpf{0}%
\ifnum\pgfutil@tmpde=11\relax%
 \expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@B@#1\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#2\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@line@A@#1\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpd{\csname tikz@td@line@A@#2\endcsname}%
\edef\pgfutil@tmpf{3}%
\else
\ifnum\pgfutil@tmpde=21\relax%
 \expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#2\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#2\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpn{\csname tikz@td@plane@normal@#1\endcsname}%
 \expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@plane@point@#1\endcsname}%
 \edef\pgfutil@tmpf{1}%
 \else
  \ifnum\pgfutil@tmpde=12\relax%
   \expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#1\endcsname}%
   \expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#1\endcsname}%
   \expandafter\edef\expandafter\pgfutil@tmpn{\csname tikz@td@plane@normal@#2\endcsname}%
   \expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@plane@point@#2\endcsname}%
   \edef\pgfutil@tmpf{1}%
  \else
   \ifnum\pgfutil@tmpde=13\relax%
	\expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#1\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#1\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@sphere@C@#2\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpr{\csname tikz@td@sphere@r@#2\endcsname}%
	\edef\pgfutil@tmpf{2}%
	%
   \else
	\ifnum\pgfutil@tmpde=31\relax%
	\expandafter\edef\expandafter\pgfutil@tmpa{\csname tikz@td@line@A@#2\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpb{\csname tikz@td@line@B@#2\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpc{\csname tikz@td@sphere@C@#1\endcsname}%
	\expandafter\edef\expandafter\pgfutil@tmpr{\csname tikz@td@sphere@r@#1\endcsname}%
	\edef\pgfutil@tmpf{2}%
    %
	\else
	 \PackageWarning{3dtools}{Currently, one intersection object has to be a plane and the other 
  	   one a line. However, #1 has dimension \pgfutil@tmpd\space and 
	   #2 has dimension \pgfutil@tmpe.}%
	\fi
   \fi	
  \fi
 \fi
\fi
\ifnum\pgfutil@tmpf=1\relax%
%
\pgfmathsetmacro{\pgfutil@tmpg}{TD("(\pgfutil@tmpn)o(\pgfutil@tmpb)-(\pgfutil@tmpa)")}%
\pgfmathtruncatemacro{\pgfutil@tmph}{abs(\pgfutil@tmpg)>0.01?1:0}%
\ifnum\pgfutil@tmph=1\relax%
\pgfmathsetmacro{\pgfutil@tmpi}{TD("(\pgfutil@tmpn)o(\pgfutil@tmpc)-(\pgfutil@tmpa)")/\pgfutil@tmpg}%
\pgfmathsetmacro{\pgfutil@tmpj}{TD("(\pgfutil@tmpa)+\pgfutil@tmpi*(\pgfutil@tmpb)-\pgfutil@tmpi*(\pgfutil@tmpa)")}%
\tikzset{insert path={(\pgfutil@tmpj)}}%
%
\else
\PackageWarning{3dtools}{The plane and line do not intersect within the uncertainties. Returning (0,0,0) instead.}%
\fi
\fi
\ifnum\pgfutil@tmpf=2\relax%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpg}{TD("(\pgfutil@tmpb)-(\pgfutil@tmpa)o(\pgfutil@tmpb)-(\pgfutil@tmpa)")}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmph}{2*TD("(\pgfutil@tmpa)-(\pgfutil@tmpc)o(\pgfutil@tmpb)-(\pgfutil@tmpa)")}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpi}{TD("(\pgfutil@tmpa)-(\pgfutil@tmpc)o(\pgfutil@tmpa)-(\pgfutil@tmpc)")-\pgfutil@tmpr*\pgfutil@tmpr}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpj}{sign(\pgfutil@tmph*\pgfutil@tmph-4*\pgfutil@tmpg*\pgfutil@tmpi)}%
\ifdim\pgfutil@tmpj pt<0pt\relax
\PackageWarning{3dtools}{The sphere and line do not intersect within the uncertainties. Returning (0,0,0) instead.}%
\else
\pgfmathsetmacro@td@FPU{\pgfutil@tmpk}{-1*(\pgfutil@tmph+sqrt(\pgfutil@tmph*\pgfutil@tmph-4*\pgfutil@tmpg*\pgfutil@tmpi))/2/\pgfutil@tmpg}%
%
\edef\pgfutil@tmpm{0}%
\ifdim\pgfutil@tmpk pt>0pt\relax
 \ifdim\pgfutil@tmpk pt<1pt\relax
  \edef\pgfutil@tmpm{1}%
  \pgfmathsetmacro{\pgfutil@tmpn}{TD("(\pgfutil@tmpa)+\pgfutil@tmpk*(\pgfutil@tmpb)-\pgfutil@tmpk*(\pgfutil@tmpa)")}%
  \tikzset{insert path={(\pgfutil@tmpn) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 1})}}%
  %
 \fi
\fi
\pgfmathsetmacro@td@FPU{\pgfutil@tmpk}{-1*(\pgfutil@tmph-sqrt(\pgfutil@tmph*\pgfutil@tmph-4*\pgfutil@tmpg*\pgfutil@tmpi))/2/\pgfutil@tmpg}%
%
\ifdim\pgfutil@tmpk pt>0pt\relax
 \ifdim\pgfutil@tmpk pt<1pt\relax
  \pgfmathsetmacro{\pgfutil@tmpn}{TD("(\pgfutil@tmpa)+\pgfutil@tmpk*(\pgfutil@tmpb)-\pgfutil@tmpk*(\pgfutil@tmpa)")}%
  \ifnum\pgfutil@tmpm=1
   \tikzset{insert path={(\pgfutil@tmpn) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 2})}}%
  \else
   \tikzset{insert path={(\pgfutil@tmpn) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 1})}}%
  \fi
 \fi
\fi
%
\fi
\fi
\ifnum\pgfutil@tmpf=3\relax%
 \pgfmathsetmacro{\pgfutil@tmpC}{TD("(\pgfutil@tmpc)")}%
 \pgfmathsetmacro{\pgfutil@tmpD}{TD("(\pgfutil@tmpd)")}%
 \pgfmathsetmacro{\pgfutil@tmpi}{sqrt(TD("(\pgfutil@tmpC)-(\pgfutil@tmpD)o(\pgfutil@tmpC)-(\pgfutil@tmpD)"))}%
 \ifdim\pgfutil@tmpi pt<0.05pt\relax
  \tikzset{insert path={(\pgfutil@tmpC) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 1})}}%
 \else
  \pgfmathsetmacro{\pgfutil@tmpE}{TD("(\pgfutil@tmpc)-(\pgfutil@tmpa)")}%
  \pgfmathsetmacro{\pgfutil@tmpF}{TD("(\pgfutil@tmpd)-(\pgfutil@tmpb)")}%
  \pgfmathsetmacro{\pgfutil@tmpG}{TD("(\pgfutil@tmpD)-(\pgfutil@tmpC)")}%
  \pgfmathsetmacro{\pgfutil@tmpH}{TD("(\pgfutil@tmpF)x(\pgfutil@tmpG)")}%
  \pgfmathsetmacro{\pgfutil@tmpK}{TD("(\pgfutil@tmpF)x(\pgfutil@tmpE)")}%
  \pgfmathsetmacro@td@FPU{\pgfutil@tmph}{sqrt(TD("(\pgfutil@tmpH)o(\pgfutil@tmpH)"))}%
  \pgfmathsetmacro@td@FPU{\pgfutil@tmpk}{sqrt(TD("(\pgfutil@tmpK)o(\pgfutil@tmpK)"))}%
  \ifdim\pgfutil@tmph pt<0.01pt\relax
   \PackageWarning{3dtools}{The lines do not intersect within the uncertainties. Returning (0,0,0) instead.}%
  \else
   \ifdim\pgfutil@tmpk pt<0.01pt\relax
	\PackageWarning{3dtools}{The lines do not intersect within the uncertainties. Returning (0,0,0) instead.}%
   \else
	\pgfmathsetmacro@td@FPU{\pgfutil@tmpl}{sign(TD("(\pgfutil@tmpH)o(\pgfutil@tmpK)"))*\pgfutil@tmph/\pgfutil@tmpk}%
	\pgfmathsetmacro{\pgfutil@tmpM}{TD("(\pgfutil@tmpC)+\pgfutil@tmpl*(\pgfutil@tmpE)")}%
	\tikzset{insert path={(\pgfutil@tmpM) coordinate (\pgfkeysvalueof{/tikz/3d/aux keys/intersection 1})}}%
   \fi 
  \fi
 \fi
\fi
}}
%
%
\tikzset{3d/circumsphere center/.code={%
\tikzset{3d/aux keys/.cd,#1}%
\edef\pgfutil@tmpA{\pgfkeysvalueof{/tikz/3d/aux keys/A}}%
\edef\pgfutil@tmpB{\pgfkeysvalueof{/tikz/3d/aux keys/B}}%
\edef\pgfutil@tmpC{\pgfkeysvalueof{/tikz/3d/aux keys/C}}%
\edef\pgfutil@tmpD{\pgfkeysvalueof{/tikz/3d/aux keys/D}}%
%
\pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfutil@tmpB-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfutil@tmpC-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpD}{TD("\pgfutil@tmpD-\pgfutil@tmpA")}%
%
\pgfmathsetmacro{\pgfutil@tmpBxC}{TD("(\pgfutil@tmpB)x(\pgfutil@tmpC)")}%
\pgfmathsetmacro{\pgfutil@tmpCxD}{TD("(\pgfutil@tmpC)x(\pgfutil@tmpD)")}%
\pgfmathsetmacro{\pgfutil@tmpDxB}{TD("(\pgfutil@tmpD)x(\pgfutil@tmpB)")}%
%
\pgfmathsetmacro{\pgfutil@tmpd}{2*TD("(\pgfutil@tmpB)o(\pgfutil@tmpCxD)")}%
%
\pgfmathtruncatemacro{\pgfutil@tmpi}{abs(\pgfutil@tmpd)>0.02?1:0}%
\ifnum\pgfutil@tmpi=0\relax
\PackageWarning{3dtools}{The points approximately sit on a common plane. The circumsphere cannot
be determined.}%
\else
\pgfmathsetmacro{\pgfutil@tmpnB}{TD("(\pgfutil@tmpB)o(\pgfutil@tmpB)")/\pgfutil@tmpd}%
\pgfmathsetmacro{\pgfutil@tmpnC}{TD("(\pgfutil@tmpC)o(\pgfutil@tmpC)")/\pgfutil@tmpd}%
\pgfmathsetmacro{\pgfutil@tmpnD}{TD("(\pgfutil@tmpD)o(\pgfutil@tmpD)")/\pgfutil@tmpd}%
\pgfmathsetmacro{\pgfutil@tmpI}{TD("\pgfutil@tmpA+\pgfutil@tmpnB*(\pgfutil@tmpCxD)+\pgfutil@tmpnC*(\pgfutil@tmpDxB)+\pgfutil@tmpnD*(\pgfutil@tmpBxC)")}%
\tikzset{insert path={(\pgfutil@tmpI)}}%
\fi
}}%
\tikzset{3d/circumcircle center/.code={%
\tikzset{3d/aux keys/.cd,#1}%
\edef\pgfutil@tmpA{\pgfkeysvalueof{/tikz/3d/aux keys/A}}%
\edef\pgfutil@tmpB{\pgfkeysvalueof{/tikz/3d/aux keys/B}}%
\edef\pgfutil@tmpC{\pgfkeysvalueof{/tikz/3d/aux keys/C}}%
%
\pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfutil@tmpB-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfutil@tmpC-\pgfutil@tmpA")}%
%
%
\pgfmathsetmacro{\pgfutil@tmpBB}{TD("(\pgfutil@tmpB)o(\pgfutil@tmpB)")}%
\pgfmathsetmacro{\pgfutil@tmpBC}{TD("(\pgfutil@tmpB)o(\pgfutil@tmpC)")}%
\pgfmathsetmacro{\pgfutil@tmpCC}{TD("(\pgfutil@tmpC)o(\pgfutil@tmpC)")}%
%
%
\pgfmathparse@td@FPU{2*(\pgfutil@tmpBB*\pgfutil@tmpCC-\pgfutil@tmpBC*\pgfutil@tmpBC)}%
\let\pgfutil@tmpd\pgfmathresult%
%
%
\pgfmathparse@td@FPU{int(abs(\pgfutil@tmpd)>0.02?1:0)}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{\pgfmathresult}%
%
\ifnum\pgfutil@tmpi=0\relax
\PackageWarning{3dtools}{The points approximately sit on a common line. The circumcircle cannot
be determined.}%
\else
%
\pgfmathparse@td@FPU{(\pgfutil@tmpBB-\pgfutil@tmpBC)*\pgfutil@tmpCC/\pgfutil@tmpd}%
\let\pgfutil@tmpb\pgfmathresult
%
%
\pgfmathparse@td@FPU{(\pgfutil@tmpCC-\pgfutil@tmpBC)*\pgfutil@tmpBB/\pgfutil@tmpd}%
\let\pgfutil@tmpc\pgfmathresult
%
%
\pgfmathsetmacro{\pgfutil@tmpI}{TD("\pgfutil@tmpA+\pgfutil@tmpb*(\pgfutil@tmpB)+\pgfutil@tmpc*(\pgfutil@tmpC)")}%
%
\tikzset{insert path={(\pgfutil@tmpI)}}%
\fi
}}%
\tikzset{3d/define orthonormal dreibein/.code={%
\tikzset{3d/aux keys/.cd,#1}%
\edef\pgfutil@tmpA{\pgfkeysvalueof{/tikz/3d/aux keys/A}}%
\edef\pgfutil@tmpB{\pgfkeysvalueof{/tikz/3d/aux keys/B}}%
\edef\pgfutil@tmpC{\pgfkeysvalueof{/tikz/3d/aux keys/C}}%
\pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfutil@tmpB-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfutil@tmpC-\pgfutil@tmpA")}%
\pgfmathsetmacro{\pgfutil@tmpD}{TD("(\pgfutil@tmpB)x(\pgfutil@tmpC)")}%
\pgfmathsetmacro@td@FPU{\pgfutil@tmpd}{min(1,TD("(\pgfutil@tmpD)o(\pgfutil@tmpD)"))}%
\ifdim\pgfutil@tmpd pt<0.01pt\relax
\PackageWarning{3dtools}{The vectors \pgfutil@tmpA, \pgfutil@tmpB\space and 
\pgfutil@tmpC are too collinear. Cannot determine appropriate plane.}%
\else
\pgfmathsetmacro{\pgfutil@tmpB}{TDunit("(\pgfutil@tmpB)")}%
\pgfmathsetmacro{\pgfutil@tmpD}{TDunit("(\pgfutil@tmpD)")}%
\pgfmathsetmacro{\pgfutil@tmpC}{TD("(\pgfutil@tmpD)x(\pgfutil@tmpB)")}%
%
%
%
\expanded{\noexpand\path[overlay,
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\pgfutil@tmpB)},
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\pgfutil@tmpC)},
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ez}=(\pgfutil@tmpD)}];}%
\fi
},3d/aux keys/.cd,A/.initial={(A)},B/.initial={(B)},
C/.initial={(C)},D/.initial={(D)},
intersection 1/.initial={I-1},intersection 2/.initial={I-2},
ex/.initial={(ex)},
ey/.initial={(ey)},ez/.initial={(ez)},
i1/.initial=i1,i2/.initial=i2,
rA/.initial=1,rB/.initial=1,rC/.initial=1,
tmpcoord1/.initial=3dtoolstmp-1}
\tikzset{3d/screen coords/.style={x={(1cm,0cm)},y={(0cm,1cm)},z={(-1cm,-1cm)}}}%
%
%
\makeatletter
\tikzset{pics/3d/dim line/.style={code={%
  \tikzset{3d/dim line/.cd,#1}%
  \pgfmathsetmacro{\pgfutil@tmpa}{tddistance("\pgfkeysvalueof{/tikz/3d/dim line/A}","\pgfkeysvalueof{/tikz/3d/dim line/B}")}%
  \ifdim\pgfutil@tmpa pt<0.02pt\relax 
   \message{The points A=\pgfkeysvalueof{/tikz/3d/dim line/A} and B=\pgfkeysvalueof{/tikz/3d/dim line/B} are too close. Cannot draw dim line.}%
  \else 
    \pgfmathsetmacro{\pgfutil@tmpa}{TD("\pgfkeysvalueof{/tikz/3d/dim line/A}-\pgfkeysvalueof{/tikz/3d/dim line/B}x\pgfkeysvalueof{/tikz/3d/dim line/n}")}%
    \pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpa)o(\pgfutil@tmpa)")}%
    \ifdim\pgfutil@tmpb pt<0.02pt\relax
      \message{The normal n=\pgfkeysvalueof{/tikz/3d/dim line/n} is either too short or too collinear with A-B=\pgfkeysvalueof{/tikz/3d/dim line/A}-\pgfkeysvalueof{/tikz/3d/dim line/B}. Cannot draw dim line.}%
    \else 
      %
      %
      %
      %
      %
      %
      %
      %
      %
      %
      %
      \pgfmathsetmacro{\pgfutil@tmpa}{TDunit("(\pgfutil@tmpa)")}%
      \pgfmathsetmacro{\pgfutil@tmpb}{\pgfkeysvalueof{/tikz/3d/dim line/d}/1cm}%
      \pgfmathsetmacro{\pgfutil@tmpex}{TDunit("\pgfkeysvalueof{/tikz/3d/dim line/B}-\pgfkeysvalueof{/tikz/3d/dim line/A}")}%
      \expanded{\noexpand\path[overlay]
        (\pgfutil@tmpex) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ex);}
      \pgfmathtruncatemacro{\pgfutil@tmpf}{ifthenelse(x2d("\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ex")<0,1,0)}%
      \ifnum\pgfutil@tmpf=1\relax 
        \pgfmathsetmacro{\pgfutil@tmpex}{TDunit("\pgfkeysvalueof{/tikz/3d/dim line/A}-\pgfkeysvalueof{/tikz/3d/dim line/B}")}%
      \fi
      \pgfmathsetmacro{\pgfutil@tmpey}{TDunit("\pgfkeysvalueof{/tikz/3d/dim line/n}x(\pgfutil@tmpex)")}%
      \expanded{\noexpand\path[overlay]
        (\pgfutil@tmpey) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ey);}
      \pgfmathtruncatemacro{\pgfutil@tmpf}{ifthenelse(y2d("\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ey")<0,1,0)}%
      \ifnum\pgfutil@tmpf=1\relax 
        \pgfmathsetmacro{\pgfutil@tmpey}{TDunit("(\pgfutil@tmpex)x\pgfkeysvalueof{/tikz/3d/dim line/n}")}%
      \fi
      \pgfmathsetmacro{\pgfutil@tmpez}{TDunit("\pgfkeysvalueof{/tikz/3d/dim line/n}")}%
      \pgfmathsetmacro{\pgfutil@tmpA}{TD("\pgfkeysvalueof{/tikz/3d/dim line/A}+\pgfutil@tmpb*(\pgfutil@tmpa)")}%
      \pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfkeysvalueof{/tikz/3d/dim line/B}+\pgfutil@tmpb*(\pgfutil@tmpa)")}%
      \pgfmathsetmacro{\pgfutil@tmpC}{TD("0.5*\pgfkeysvalueof{/tikz/3d/dim line/A}+0.5*\pgfkeysvalueof{/tikz/3d/dim line/B}+\pgfutil@tmpb*(\pgfutil@tmpa)")}%
      \expanded{\noexpand\path[overlay]
      %
      (\pgfutil@tmpex) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ex)
      (\pgfutil@tmpey) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ey)
      (\pgfutil@tmpez) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ez)
      (\pgfutil@tmpA) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}A')
      (\pgfutil@tmpB) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}B')
      (\pgfutil@tmpC) coordinate (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}AB')
      ;}%
      \begin{scope}[x={(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ex)},
          y={(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ey)},
          z={(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}ez)},canvas is xy plane at z=0]          
          \path (\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}AB') node[3d/dim line/dim label](\pgfkeysvalueof{/tikz/3d/dim line/node name}){\tikz@td@dim@line@label};
          \fill let \p1=($(\pgfkeysvalueof{/tikz/3d/dim line/node name}.west)-(\pgfkeysvalueof{/tikz/3d/dim line/node name}.east)$),\n1={0.5*sqrt((\x1)*(\x1)+(\y1)*(\y1))},\p2=($(\pgfkeysvalueof{/tikz/3d/dim line/node name})-(\pgfkeysvalueof{/tikz/3d/dim line/auxiliary coordinate prefix}A')$),\n2={sqrt((\x2)*(\x2)+(\y2)*(\y2))-\n1-0.4pt} in (\pgfkeysvalueof{/tikz/3d/dim line/node name}) ++ (\n1,0) -- ++ (0,0.2pt) -- ++ (\n2-3pt,0pt)
          -- ++ (0pt,1.3pt) -- ++ (3pt,-1.5pt) -- ++ (-3pt,-1.5pt)  -- ++ (0pt,1.3pt) -- ++ (3pt-\n2,0pt) -- cycle
          (\pgfkeysvalueof{/tikz/3d/dim line/node name}) ++ (-\n1,0) -- ++ (0,-0.2pt) -- ++ (3pt-\n2,0pt)
          -- ++ (0pt,-1.3pt) -- ++ (-3pt,1.5pt) -- ++ (3pt,1.5pt)  -- ++ (0pt,-1.3pt) -- ++ (\n2-3pt,0pt) -- cycle
          (\pgfkeysvalueof{/tikz/3d/dim line/node name}) ++ (\n1+\n2,1.5pt) -- ++ (0.4pt,0pt) -- ++ (0pt,-3pt) -- ++ (-0.4pt,0pt) -- cycle
          (\pgfkeysvalueof{/tikz/3d/dim line/node name}) ++ (0pt-\n1-\n2,-1.5pt) -- ++ (-0.4pt,0pt) -- ++ (0pt,3pt) -- ++ (0.4pt,0pt) -- cycle;
      \end{scope}
    \fi 
  \fi  
}},3d/dim line/.cd,A/.initial={(0,0,0)},B/.initial={(1,0,0)},n/.initial={(0,0,1)},
l/.store in=\tikz@td@dim@line@label,
l=\empty,
auxiliary coordinate prefix/.initial=tmp,d/.initial=2mm,
dim label/.style={transform shape,circle,inner sep=1pt},
node name/.initial=dim label}
%
\tikzset{pics/3d circle through 3 points/.style={code={%
 \tikzset{3d/circle through 3 points/.cd,#1}%
 \expanded{\noexpand\path[overlay,
3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)=\pgfkeysvalueof{/tikz/3d/circle through 3 points/A}-\pgfkeysvalueof{/tikz/3d/circle through 3 points/C}},
 3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)=\pgfkeysvalueof{/tikz/3d/circle through 3 points/B}-\pgfkeysvalueof{/tikz/3d/circle through 3 points/C}},
 3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)=\pgfkeysvalueof{/tikz/3d/circle through 3 points/A}-\pgfkeysvalueof{/tikz/3d/circle through 3 points/B}},
 3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)=(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)x(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)}
 ];}%
 \pgfmathsetmacro@td@FPU{\lengthn}{sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)"))}
 \ifdim\lengthn pt<0.02pt\relax
   \message{The points are (almost) on a line. Circle cannot be determined.}
  \else
   \pgfmathsetmacro@td@FPU{\tmpradius}{sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)"))*%
   	sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)"))*sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)"))/%
		(2*\lengthn)}
   \pgfmathsetmacro@td@FPU{\coeffa}{-1*TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)")/(2*TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)"))}		
   \pgfmathsetmacro@td@FPU{\coeffb}{TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)")/(2*TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)"))}
   \expanded{%
   \noexpand\path[overlay,3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}u)=\coeffa*(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)x(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)},
     3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}v)=\coeffb*(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}b)x(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)}];
   \noexpand\path[3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/center name})=\pgfkeysvalueof{/tikz/3d/circle through 3 points/C}+(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}u)+(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}v)}];
   }%
   \pgfmathsetmacro{\normalizationa}{1/sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)"))}
   \pgfmathsetmacro{\normalizationn}{1/sqrt(TD("(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)o(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)"))}
   \expanded{%
   \noexpand\path[overlay,3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)=\normalizationa*(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)},
   3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)=\normalizationn*(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)},
   3d coordinate={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)=(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)x(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}n)}];
   }%
   \expanded{%
	\noexpand\begin{scope}[plane x={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}a)},plane y={(\pgfkeysvalueof{/tikz/3d/circle through 3 points/auxiliary coordinate prefix}c)},canvas is plane]
	 \noexpand\draw[pic actions] (\pgfkeysvalueof{/tikz/3d/circle through 3 points/center name}) circle[radius=\tmpradius];
	 \noexpand\pgfkeys{/tikz/3d/circle through 3 points/extra}
	\noexpand\end{scope}}%
  \fi 
}},3d/circle through 3 points/.cd,A/.initial={(1,0,0)},B/.initial={(0,1,0)},
C/.initial={(0,0,1)},
auxiliary coordinate prefix/.initial=tmp,center name/.initial=M,
extra/.code={}}%
%
%
\tikzset{pics/3d incircle/.style={code={%
\tikzset{3d/incircle/.cd,#1}%
\pgfmathsetmacro{\pgfutil@tmpa}{tddistance("\pgfkeysvalueof{/tikz/3d/incircle/B}","\pgfkeysvalueof{/tikz/3d/incircle/C}")}%
\pgfmathsetmacro{\pgfutil@tmpb}{tddistance("\pgfkeysvalueof{/tikz/3d/incircle/A}","\pgfkeysvalueof{/tikz/3d/incircle/C}")}%
\pgfmathsetmacro{\pgfutil@tmpc}{tddistance("\pgfkeysvalueof{/tikz/3d/incircle/A}","\pgfkeysvalueof{/tikz/3d/incircle/B}")}%
\pgfmathsetmacro{\pgfutil@tmpd}{(\pgfutil@tmpa+\pgfutil@tmpb+\pgfutil@tmpc)/2}%
\pgfmathsetmacro{\pgfutil@tmparea}{sqrt(\pgfutil@tmpd*(\pgfutil@tmpd-\pgfutil@tmpa)*(\pgfutil@tmpd-\pgfutil@tmpb)*(\pgfutil@tmpd-\pgfutil@tmpc))}%
\pgfmathsetmacro{\pgfutil@tmpr}{\pgfutil@tmparea/\pgfutil@tmpd}%
%
%
\expanded{\noexpand\tikz@td@parse@coord\pgfkeysvalueof{/tikz/3d/incircle/A}}%
\pgfmathsetmacro{\pgfutil@tmp@Ax}{\pgf@X}%
\pgfmathsetmacro{\pgfutil@tmp@Ay}{\pgf@Y}%
\pgfmathsetmacro{\pgfutil@tmp@Az}{\pgf@Z}%
%
%
\expanded{\noexpand\tikz@td@parse@coord\pgfkeysvalueof{/tikz/3d/incircle/B}}%
\pgfmathsetmacro{\pgfutil@tmp@Bx}{\pgf@X}%
\pgfmathsetmacro{\pgfutil@tmp@By}{\pgf@Y}%
\pgfmathsetmacro{\pgfutil@tmp@Bz}{\pgf@Z}%
%
%
\expanded{\noexpand\tikz@td@parse@coord\pgfkeysvalueof{/tikz/3d/incircle/C}}%
\pgfmathsetmacro{\pgfutil@tmp@Cx}{\pgf@X}%
\pgfmathsetmacro{\pgfutil@tmp@Cy}{\pgf@Y}%
\pgfmathsetmacro{\pgfutil@tmp@Cz}{\pgf@Z}%
\pgfmathsetmacro{\pgfutil@tmpIx}{\pgfutil@tmp@Ax*\pgfutil@tmpa+\pgfutil@tmp@Bx*\pgfutil@tmpb+\pgfutil@tmp@Cx*\pgfutil@tmpc)/\pgfutil@tmpd/2}%
\pgfmathsetmacro{\pgfutil@tmpIy}{\pgfutil@tmp@Ay*\pgfutil@tmpa+\pgfutil@tmp@By*\pgfutil@tmpb+\pgfutil@tmp@Cy*\pgfutil@tmpc)/\pgfutil@tmpd/2}%
\pgfmathsetmacro{\pgfutil@tmpIz}{\pgfutil@tmp@Az*\pgfutil@tmpa+\pgfutil@tmp@Bz*\pgfutil@tmpb+\pgfutil@tmp@Cz*\pgfutil@tmpc)/\pgfutil@tmpd/2}%
\path (\pgfutil@tmpIx,\pgfutil@tmpIy,\pgfutil@tmpIz) 
  coordinate (\pgfkeysvalueof{/tikz/3d/incircle/center name})
  [3d/projection of={(\pgfkeysvalueof{/tikz/3d/incircle/center name}) on 
	\pgfkeysvalueof{/tikz/3d/incircle/A}--\pgfkeysvalueof{/tikz/3d/incircle/B}}] 
 coordinate (\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}c)
 [3d/projection of={(\pgfkeysvalueof{/tikz/3d/incircle/center name}) on 
	\pgfkeysvalueof{/tikz/3d/incircle/A}--\pgfkeysvalueof{/tikz/3d/incircle/C}}] 
 coordinate (\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}b)
 [3d/projection of={(\pgfkeysvalueof{/tikz/3d/incircle/center name}) on 
	\pgfkeysvalueof{/tikz/3d/incircle/B}--\pgfkeysvalueof{/tikz/3d/incircle/C}}] 
 coordinate (\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}a);
 \path[pic actions] pic{3d circle through 3 points={%
   	A={(\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}c)},%
   	B={(\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}b)},%
  	C={(\pgfkeysvalueof{/tikz/3d/incircle/projection prefix}a)},%
  	center name=\pgfkeysvalueof{/tikz/3d/incircle/center name}}}
	;
}},3d/incircle/.cd,
center name/.initial=I,
A/.initial={(1,0,0)},B/.initial={(0,1,0)},C/.initial={(0,0,1)},
projection prefix/.initial=tmpp}
%
\tikzset{pics/3d/circle on sphere/.style={code={%
 \tikzset{3d/circle on sphere/.cd,#1}%
 \edef\pgfutil@tmpR{\pgfkeysvalueof{/tikz/3d/circle on sphere/R}}%
 \edef\pgfutil@tmpC{\pgfkeysvalueof{/tikz/3d/circle on sphere/C}}%
 \edef\pgfutil@tmpP{\pgfkeysvalueof{/tikz/3d/circle on sphere/P}}%
 \edef\pgfutil@tmpn{\pgfkeysvalueof{/tikz/3d/circle on sphere/n}}%
 \edef\pgfutil@tmpPname{\pgfkeysvalueof{/tikz/3d/circle on sphere/auxiliary coordinate prefix}P}%
 \pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfutil@tmpC")}%
 \pgfmathsetmacro{\pgfutil@tmpP}{TD("\pgfutil@tmpP")}%
 \pgfmathsetmacro{\pgfutil@tmpn}{TD("\pgfutil@tmpn")}%
 \pgfmathsetmacro{\pgfutil@tmpd}{sqrt(TD("(\pgfutil@tmpP)-(\pgfutil@tmpC)o(\pgfutil@tmpP)-(\pgfutil@tmpC)"))}%
 \ifdim\pgfutil@tmpd pt>0.02pt\relax
  %
  \pgfmathsetmacro{\pgfutil@tmpn}{TD("(\pgfutil@tmpP)-(\pgfutil@tmpC)")}%
 \fi
 %
 \pgfmathsetmacro{\pgfutil@tmpa}{sqrt(TD("(\pgfutil@tmpn)o(\pgfutil@tmpn)"))}%
 \ifdim\pgfutil@tmpa pt<0.02pt\relax
  \PackageWarning{3dtools}{Chosen normal is too short.}%
 \else
 \pgfmathtruncatemacro{\pgfutil@tmpb}{(\pgfutil@tmpd<\pgfutil@tmpR?1:0)} 
 \ifnum\pgfutil@tmpb=0
  \PackageWarning{3dtools}{Circle center is not inside the sphere.}
 \else 
  \pgfmathsetmacro{\pgfutil@tmpr}{sqrt(\pgfutil@tmpR*\pgfutil@tmpR-\pgfutil@tmpd*\pgfutil@tmpd)}%
  \pgfmathsetmacro{\pgfutil@tmpa}{1/\pgfutil@tmpa}%
  \pgfmathsetmacro{\pgfutil@tmpz}{TD("\pgfutil@tmpa*(\pgfutil@tmpn)")}%
  \path[overlay] (nscreenx,nscreeny,nscreenz) coordinate (nscreen)
	[3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ez}=(\pgfutil@tmpz)},
	3d coordinate/.expanded={(\pgfutil@tmpPname)=(\pgfutil@tmpP)}];%
  \pgfmathsetmacro{\pgfutil@tmpy}{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ez}x(nscreen)")}%
  \pgfmathsetmacro{\pgfutil@tmpa}{sqrt(TD("(\pgfutil@tmpy)o(\pgfutil@tmpy)"))}%
  \ifdim\pgfutil@tmpa pt<0.04pt%
   %
   \pgfmathsetmacro{\pgfutil@tmpx}{normalcandidate(\pgfutil@tmpz)}%
   \pgfmathsetmacro{\pgfutil@tmpy}{TD("(\pgfutil@tmpz)x(\pgfutil@tmpx)")}
   \path[overlay] 
	[3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\pgfutil@tmpx)},
	 3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\pgfutil@tmpy)}];
   \pgfmathtruncatemacro{\pgfutil@tmpa}{(TD("\pgfkeysvalueof{/tikz/3d/aux keys/ez}o(\pgfutil@tmpn)")<0?0:1)}%
   \begin{scope}[x/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}},%
   	y/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}},%
	z/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ez}},%
	shift={(\pgfutil@tmpPname)}]
	\ifcase\pgfutil@tmpa
	 %
	 \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/back layer}}%
	  \draw[3d/hidden]  circle[radius=\pgfutil@tmpr];
	 \end{pgfonlayer}%
	\or
	 %
	 \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/fore layer}}%
	  \draw[3d/visible] circle[radius=\pgfutil@tmpr];
	 \end{pgfonlayer}%
	\fi
   \end{scope}
  \else%
   \pgfmathsetmacro{\pgfutil@tmpa}{1/\pgfutil@tmpa}%
   \pgfmathsetmacro{\pgfutil@tmpy}{TD("\pgfutil@tmpa*(\pgfutil@tmpy)")}%
   \pgfmathsetmacro{\pgfutil@tmpx}{TD("(\pgfutil@tmpy)x(\pgfutil@tmpz)")}%
   \pgfmathsetmacro{\pgfutil@tmps}{TD("(nscreen)")}%
   \pgfmathsetmacro{\pgfutil@tmpp}{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ez}o(nscreen)")}%
   \pgfmathsetmacro{\pgfutil@tmpo}{sqrt(1-\pgfutil@tmpp*\pgfutil@tmpp)}%
   \pgfmathsetmacro{\pgfutil@tmpa}{atan2(-1*\pgfutil@tmpp,\pgfutil@tmpo)}%
   \pgfmathsetmacro{\pgfutil@tmpb}{screendepth(\pgfutil@tmpP)}%
   \pgfmathsetmacro{\pgfutil@tmpc}{screendepth(\pgfutil@tmpC)}%
   \path[overlay,
		3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\pgfutil@tmpx)},
		3d coordinate/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\pgfutil@tmpy)}];%
%
%
%
   \begin{scope}[x/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}},%
   	 y/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}},%
	 z/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ez}},%
	 shift={(\pgfutil@tmpPname)}]  
    \pgfmathtruncatemacro{\pgfutil@tmpi}{(abs(\pgfutil@tmpr*cos(\pgfutil@tmpa))>abs(\pgfutil@tmpb-\pgfutil@tmpc)?1:0)}%
 	\ifcase\pgfutil@tmpi
%
 	 \pgfmathtruncatemacro{\pgfutil@tmpj}{(\pgfutil@tmpb<\pgfutil@tmpc?0:1)}%
 	 \ifcase\pgfutil@tmpj
%
      \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/back layer}}%
 	   \draw[3d/hidden]  circle[radius=\pgfutil@tmpr];
	  \end{pgfonlayer}%
 	 \or
%
	  \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/fore layer}}%
 	   \draw[3d/visible]  circle[radius=\pgfutil@tmpr];
	  \end{pgfonlayer}%
 	 \fi
 	\or
%
	 \pgfmathsetmacro{\pgfutil@tmpf}{abs(acos((\pgfutil@tmpc-\pgfutil@tmpb)/\pgfutil@tmpr/cos(\pgfutil@tmpa))}%
	 \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/back layer}}%
	  \draw[3d/hidden]  (\pgfutil@tmpf:\pgfutil@tmpr) arc[start angle=\pgfutil@tmpf,
	 	end angle=360-\pgfutil@tmpf,radius=\pgfutil@tmpr];
     \end{pgfonlayer}%
	 \begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/circle on sphere/fore layer}}%
	  \draw[3d/visible]  (\pgfutil@tmpf:\pgfutil@tmpr) arc[start angle=\pgfutil@tmpf,
	 	end angle=-\pgfutil@tmpf,radius=\pgfutil@tmpr];
	 \end{pgfonlayer}%
 	\fi
   \end{scope}
   \fi	
  \fi
 \fi  
}},3d/circle on sphere/.cd,C/.initial={(0,0,0)},
	P/.initial={(0,0,0)},R/.initial=1,%
	n/.initial={(0,0,1)},auxiliary coordinate prefix/.initial=tmp,%
	fore layer/.initial=main,back layer/.initial=main}
%
\tikzset{pics/3d/cone/.style={code={%
	\tikzset{3d/.cd,#1}%
	\def\pv##1{\pgfkeysvalueof{/tikz/3d/##1}}%
	\pgfmathsetmacro{\sdtip}{screendepth(0,0,\pv{h})}
	\pgfmathsetmacro{\aspectangle}{atan2(\sdtip,sqrt(\pv{h}*\pv{h}-\sdtip*\sdtip))}
	\path (0,0,\pv{h}) coordinate (-tip);
	\pgfmathsetmacro{\myey}{TDunit("(0,0,1)x(nscreenx,nscreeny,nscreenz)")}%
	\path (0,0,{tan(\aspectangle)}) coordinate (-tmpex)
		(\myey) coordinate (-tmpey);	
    \begin{scope}[x={(-tmpex)},y={(-tmpey)}]
	 \pgfmathtruncatemacro{\itest}{abs(tan(\aspectangle)*\pv{r}/\pv{h})<1}
	 \ifnum\itest=1
	  \pgfmathsetmacro{\alphacrit}{acos(tan(\aspectangle)*\pv{r}/\pv{h})}
	  \ifdim\sdtip pt>0pt
	   \path[/tikz/3d/hidden] (\alphacrit:\pv{r}) arc[start angle=\alphacrit,end
	   angle=-\alphacrit,radius=\pv{r}];
	   \path[/tikz/3d/visible,/tikz/3d/cone/outer] (\alphacrit:\pv{r}) 
	   arc[start angle=\alphacrit,end  angle=360-\alphacrit,radius=\pv{r}]
	   -- (-tip) -- cycle;
	  \else
	   \path[/tikz/3d/visible,/tikz/3d/cone/inner] (0,0) circle[radius=\pv{r}];
	   \path[/tikz/3d/visible,/tikz/3d/cone/outer] (\alphacrit:\pv{r}) 
	   arc[start angle=\alphacrit,end  angle=-\alphacrit,radius=\pv{r}]
	   -- (-tip) -- cycle;
	  \fi
	 \else
	  \path[/tikz/3d/visible] circle[radius=\pv{r}];	 
	 \fi
    \end{scope}
	}},3d/cone/.cd,outer/.style={},inner/.style={}}
%
\tikzset{pics/3d/shaded cone/.style={code={%
	\tikzset{3d/.cd,#1}%
	\def\pv##1{\pgfkeysvalueof{/tikz/3d/##1}}%
	\pgfmathsetmacro{\sdtip}{screendepth(0,0,\pv{h})}
	\pgfmathsetmacro{\aspectangle}{atan2(\sdtip,sqrt(\pv{h}*\pv{h}-\sdtip*\sdtip))}
	\path (0,0,0) coordinate (-base) (0,0,\pv{h}) coordinate (-tip);
    \begin{scope}[x={(0,0,tan(\aspectangle))},y={($(0,0,0)!1cm!90:(0,0,\pv{h})$)}]
	 \pgfmathtruncatemacro{\itest}{abs(tan(\aspectangle)*\pv{r}/\pv{h})<1}
	 %
	 \ifnum\itest=1
	  \pgfmathsetmacro{\alphacrit}{acos(tan(\aspectangle)*\pv{r}/\pv{h})}
   	  \pgfmathtruncatemacro{\itest}{y2d("-tip")>y2d("-base")?1:0}
      \ifnum\itest=1 
	   \pgfmathsetmacro{\alphacritB}{-\alphacrit}
	   \pgfmathsetmacro{\alphacritC}{360-\alphacrit}
	  \else
	   \pgfmathsetmacro{\alphacritB}{360-\alphacrit}
	   \pgfmathsetmacro{\alphacritC}{-\alphacrit}
	  \fi
	  %
	  \ifdim\sdtip pt>0pt
	   \begin{scope}
	    \clip (\alphacrit:\pv{r}) 
	     arc[start angle=\alphacrit,end  angle=\alphacritC,radius=\pv{r}]
	     -- (-tip) -- cycle;
	    \path[3d/cone/outer shade,3d/screen coords]	
		 (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	   \path[/tikz/3d/hidden] (\alphacrit:\pv{r}) arc[start angle=\alphacrit,end
	    angle=\alphacritB,radius=\pv{r}];
	   \path[/tikz/3d/visible] (\alphacrit:\pv{r}) 
	    arc[start angle=\alphacrit,end  angle=\alphacritC,radius=\pv{r}]
	    -- (-tip) -- cycle;
	  \else
	   \begin{scope}
	    \clip (0,0) circle[radius=\pv{r}];
	    \path[3d/cone/inner shade,3d/screen coords]	
		 (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	   \path[/tikz/3d/visible,/tikz/3d/cone/inner] (0,0) circle[radius=\pv{r}];
	   \begin{scope}
	    \clip (\alphacrit:\pv{r}) 
	     arc[start angle=\alphacrit,end  angle=\alphacritB,radius=\pv{r}]
	    -- (-tip) -- cycle;
	    \path[3d/cone/outer shade,3d/screen coords]	
		 (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	   \path[/tikz/3d/visible,/tikz/3d/cone/outer] (\alphacrit:\pv{r}) 
	    arc[start angle=\alphacrit,end  angle=\alphacritB,radius=\pv{r}]
	    -- (-tip) -- cycle;
	  \fi
	 \else
      \ifdim\sdtip pt>0pt
	   \begin{scope}
		\clip (0,0) circle[radius=\pv{r}];	 
	     \path[3d/cone/outer shade,3d/screen coords]	
		  (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	  \else
	   \begin{scope}
		\clip (0,0) circle[radius=\pv{r}];	 
	     \path[3d/cone/inner shade,3d/screen coords]	
		  (-tip) circle[radius={abs(\pv{r})+abs(\pv{h})}];
	   \end{scope}
	  \fi
	  \path[/tikz/3d/visible] circle[radius=\pv{r}];	 
	 \fi
    \end{scope}
	}},3d/cone/.cd,outer shade/.style={3d/cone shading},
	inner shade/.style={3d/cone shading={brightness=0.3}}}	
%
\tikzset{pics/3d/frustum/.style={code={%
  \tikzset{3d/.cd,#1}
  \def\pv##1{\pgfkeysvalueof{/tikz/3d/##1}}%
  \pgfmathtruncatemacro{\itest}{abs(\pv{R}-\pv{r})>0.02}
  \ifnum\itest=0
   %
   \path[overlay] (0,0,0) coordinate (-tdtmpo)
	(0,0,\pv{h}) coordinate (-tdtmpez)
	($(0,0,0)!1cm!90:(0,0,\pv{h})$) coordinate (-tdtmpey);
   \pgfmathsetmacro{\mytest}{y2d("-tdtmpez")}	
   \pgfmathsetmacro@td@FPU{\pgfutil@tmpa}{sqrt(pow(x2d("-tdtmpo")-x2d("-tdtmpez"),2)+pow(y2d("-tdtmpo")-y2d("-tdtmpez"),2))}%
   \pgfmathtruncatemacro{\itest}{(\pgfutil@tmpa>0.5?1:0)}%
   \ifnum\itest=0
	\draw[3d/visible] (0,0,0) circle[radius=R];
   \else
    \pgfmathtruncatemacro{\itest}{sign(screendepth(0,0,\pv{h}))+1}%
	\pgfmathsetmacro{\sdtip}{screendepth(0,0,\pv{h})}%
	\pgfmathsetmacro{\aspectangle}{atan2(\sdtip,\pgfutil@tmpa/1cm)}%
	\path[overlay] (0,0,{tan(\aspectangle)}) coordinate (-tdtmpex);
	\begin{scope}[x={(-tdtmpex)},y={(-tdtmpey)}]
	 \ifcase\itest\relax
      %
	  \draw[3d/hidden] (-tdtmpez)+(0,\pv{r})
	  	arc[start angle=90,end angle=-90,radius=\pv{r}];
	  \draw[3d/visible]  (0,\pv{R}) 
	   -- ($(-tdtmpez)+(0,\pv{r})$) 
	   arc[start angle=90,end angle=270,radius=\pv{r}]
	   -- (0,-\pv{R})
	   (0,0) circle[radius=\pv{R}];
	 \or
      %
	  \draw[3d/visible]  (0,\pv{R}) 
	   -- ($(-tdtmpez)+(0,\pv{r})$) 
	   -- ($(-tdtmpez)+(0,-\pv{r})$) -- (0,-\pv{R}) -- cycle;
	 \or
      %
	  \draw[3d/hidden] (0,\pv{R})
	  	arc[start angle=90,end angle=-90,radius=\pv{R}];
	  \draw[3d/visible] (-tdtmpez)+ (0,\pv{r}) 
	   -- (0,\pv{R})
	   arc[start angle=90,end angle=270,radius=\pv{R}]
	   -- ($(-tdtmpez)+(0,-\pv{r})$) 
	   (-tdtmpez) circle[radius=\pv{r}];
	 \fi
	\end{scope} 
   \fi
  \else
   \pgfmathsetmacro{\myH}{(\pv{R}*\pv{h}/(\pv{R}-\pv{r}))}%
   \pgfmathsetmacro{\sdtip}{screendepth(0,0,\myH)}%
   \pgfmathsetmacro{\aspectangle}{atan2(\sdtip,sqrt(\myH*\myH-\sdtip*\sdtip))}%
   %
   \path[overlay] (0,0,\myH) coordinate (-tip)
   (0,0,\pv{h}) coordinate (-upper base)
   (0,0,{tan(\aspectangle)}) coordinate (-tdtmpex)
   ($(0,0,0)!1cm!90:(0,0,\pv{h})$) coordinate (-tdtmpey);
   \begin{scope}[x={(-tdtmpex)},y={(-tdtmpey)}]
	   \pgfmathtruncatemacro{\itest}{abs(tan(\aspectangle)*\pv{R}/\myH)<1}
	   \path[local bounding box=pft] (-upper base) circle[radius=\pv{r}]
	    (0,0,0) circle[radius=\pv{R}];
	   \ifnum\itest=1
		\pgfmathsetmacro{\alphacrit}{acos(tan(\aspectangle)*\pv{R}/\myH)}
		\ifdim\sdtip pt>0pt\relax
		 \begin{scope}
		  \clip (-upper base) circle[radius=\pv{r}] ;
		  \path[/tikz/3d/hidden] (\alphacrit:\pv{R}) arc[start angle=\alphacrit,end
		  angle=-\alphacrit,radius=\pv{R}];
		  \path[/tikz/3d/hidden] ($(-upper base)+(\alphacrit:\pv{r})$)
		  --(\alphacrit:\pv{R}) 
		  arc[start angle=\alphacrit,end  angle=360-\alphacrit,radius=\pv{R}]
		  -- ($(-upper base)+(360-\alphacrit:\pv{r})$);
		 \end{scope}
		 \begin{scope}
		  \clip[even odd clip] (-upper base) circle[radius=\pv{r}]  [generous outside path];
		  \path[/tikz/3d/hidden] (\alphacrit:\pv{R}) arc[start angle=\alphacrit,end
		  angle=-\alphacrit,radius=\pv{R}];
		  \path[/tikz/3d/visible] ($(-upper base)+(\alphacrit:\pv{r})$)
		  --(\alphacrit:\pv{R}) 
		  arc[start angle=\alphacrit,end  angle=360-\alphacrit,radius=\pv{R}]
		  -- ($(-upper base)+(360-\alphacrit:\pv{r})$);
		 \end{scope}
		 \path[/tikz/3d/visible] (-upper base) circle[radius=\pv{r}];
		\else %
		 \begin{scope}
		  \clip circle[radius=\pv{R}];
		  \path[/tikz/3d/hidden] ($(-upper base)+(\alphacrit:\pv{r})$)
		  --(\alphacrit:\pv{R}) 
		  ($(-upper base)+(360-\alphacrit:\pv{r})$)
		  --(360-\alphacrit:\pv{R});
		  \path[/tikz/3d/hidden] (-upper base) circle[radius=\pv{r}];
		 \end{scope}
%
%
%
%
%
%
		 \begin{scope}
 		  \clip[even odd clip] circle[radius=\pv{R}] [generous outside path];
		  \path[/tikz/3d/hidden]  ($(-upper base)+(\alphacrit:\pv{r})$)
		  arc[start angle=\alphacrit,end  angle=-\alphacrit,radius=\pv{r}];
		  \path[/tikz/3d/visible] (\alphacrit:\pv{R}) --
		  ($(-upper base)+(\alphacrit:\pv{r})$)
		  arc[start angle=\alphacrit,end  angle=360-\alphacrit,radius=\pv{r}]
		  --(360-\alphacrit:\pv{R});
		 \end{scope}
		 \path[/tikz/3d/visible] circle[radius=\pv{R}];
		\fi
	   \else
		\path[/tikz/3d/visible] circle[radius=\pv{R}];	 
		\path[/tikz/3d/hidden] (-upper base) circle[radius=\pv{r}];
	   \fi
   \end{scope}
  \fi
}}}
%
\pgfmathdeclarefunction{tddistance}{2}{%
\begingroup%
\pgfmathparse@td@FPU{sqrt(TD("#1-#2o#1-#2"))}%
\pgfmathsmuggle\pgfmathresult\endgroup%
}%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\tikzset{3d/.cd,intersection of three spheres/.code={%
\tikzset{3d/aux keys/.cd,#1,/tikz/3d/define orthonormal dreibein}%
\pgfmathsetmacro\pgfutil@tmpA{TD("\pgfkeysvalueof{/tikz/3d/aux keys/A}")}%
\pgfmathsetmacro\pgfutil@tmpB{TD("\pgfkeysvalueof{/tikz/3d/aux keys/B}")}%
\pgfmathsetmacro\pgfutil@tmpC{TD("\pgfkeysvalueof{/tikz/3d/aux keys/C}")}%
\pgfmathsetmacro\pgfutil@tmpex{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ex}")}%
\pgfmathsetmacro\pgfutil@tmpey{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ey}")}%
\pgfmathsetmacro\pgfutil@tmpez{TD("\pgfkeysvalueof{/tikz/3d/aux keys/ez}")}%
\pgfmathsetmacro\pgfutil@tmpAB{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)")}%
\pgfmathsetmacro\pgfutil@tmpd{sqrt(TD("(\pgfutil@tmpAB)o(\pgfutil@tmpAB)"))}%
\ifdim\pgfutil@tmpd pt<0.1pt\relax
\PackageWarning{3dtools}{Points \pgfkeysvalueof{/tikz/3d/aux keys/A} and \pgfkeysvalueof{/tikz/3d/aux keys/B} are too close to each other.}%
\else
\pgfmathsetmacro\pgfutil@tmpAC{TD("(\pgfutil@tmpC)-(\pgfutil@tmpA)")}%
%
\pgfmathsetmacro\pgfutil@tmpi{TD("(\pgfutil@tmpex)o(\pgfutil@tmpAC)")}%
%
\pgfmathsetmacro\pgfutil@tmpj{TD("(\pgfutil@tmpey)o(\pgfutil@tmpAC)")}%
\edef\pgfutil@tmprA{\pgfkeysvalueof{/tikz/3d/aux keys/rA}}%
\edef\pgfutil@tmprB{\pgfkeysvalueof{/tikz/3d/aux keys/rB}}%
\edef\pgfutil@tmprC{\pgfkeysvalueof{/tikz/3d/aux keys/rC}}%
%
\pgfmathsetmacro\pgfutil@tmpx{(pow(\pgfutil@tmprA,2)-pow(\pgfutil@tmprB,2)%
+pow(\pgfutil@tmpd,2))/(2*(\pgfutil@tmpd))}%
%
\pgfmathsetmacro\pgfutil@tmpy{(\pgfutil@tmprA*\pgfutil@tmprA-\pgfutil@tmprC*\pgfutil@tmprC%
-2*(\pgfutil@tmpi)*(\pgfutil@tmpx)+(\pgfutil@tmpi)*(\pgfutil@tmpi)%
+(\pgfutil@tmpj)*(\pgfutil@tmpj))/(2*(\pgfutil@tmpj))}%
%
\pgfmathsetmacro\pgfutil@tmpc{\pgfutil@tmprA*\pgfutil@tmprA-pow(\pgfutil@tmpx,2)-pow(\pgfutil@tmpy,2)}%
\ifdim\pgfutil@tmpc pt<0pt\relax
\PackageWarning{3dtools}{Not all spheres intersect.}%
\else
\pgfmathsetmacro\pgfutil@tmpz{sqrt(\pgfutil@tmpc)}%
\pgfmathsetmacro\pgfutil@tmpd{TD("(\pgfutil@tmpA)+\pgfutil@tmpx*(\pgfutil@tmpex)%
+\pgfutil@tmpy*(\pgfutil@tmpey)+\pgfutil@tmpz*(\pgfutil@tmpez)")}%
\pgfmathsetmacro\pgfutil@tmpe{TD("(\pgfutil@tmpA)+\pgfutil@tmpx*(\pgfutil@tmpex)%
+\pgfutil@tmpy*(\pgfutil@tmpey)-\pgfutil@tmpz*(\pgfutil@tmpez)")}%
\tikzset{insert path={%
(\pgfutil@tmpd) coordinate(\pgfkeysvalueof{/tikz/3d/aux keys/i1}) 
(\pgfutil@tmpe) coordinate(\pgfkeysvalueof{/tikz/3d/aux keys/i2}) 
}}
\fi
\fi
}}%
%
\tikzset{3d/insphere center/.code={%
 \tikzset{3d/insphere/.cd,#1}%
 \pgfmathsetmacro{\pgfutil@tmpA}{TD("\pgfkeysvalueof{/tikz/3d/insphere/B}x\pgfkeysvalueof{/tikz/3d/insphere/C}")}%
 \pgfmathsetmacro{\pgfutil@tmpA}{sqrt(TD("(\pgfutil@tmpA)o(\pgfutil@tmpA)"))/2}%
 \pgfmathsetmacro{\pgfutil@tmpB}{TD("\pgfkeysvalueof{/tikz/3d/insphere/A}x\pgfkeysvalueof{/tikz/3d/insphere/C}")}%
 \pgfmathsetmacro{\pgfutil@tmpB}{sqrt(TD("(\pgfutil@tmpB)o(\pgfutil@tmpB)"))/2}%
 \pgfmathsetmacro{\pgfutil@tmpC}{TD("\pgfkeysvalueof{/tikz/3d/insphere/A}x\pgfkeysvalueof{/tikz/3d/insphere/B}")}%
 \pgfmathsetmacro{\pgfutil@tmpC}{sqrt(TD("(\pgfutil@tmpC)o(\pgfutil@tmpC)"))/2}%
 \pgfmathsetmacro{\pgfutil@tmpD}{TD("\pgfkeysvalueof{/tikz/3d/insphere/A}-\pgfkeysvalueof{/tikz/3d/insphere/B}x\pgfkeysvalueof{/tikz/3d/insphere/C}-\pgfkeysvalueof{/tikz/3d/insphere/B}")}%
 \pgfmathsetmacro{\pgfutil@tmpD}{sqrt(TD("(\pgfutil@tmpD)o(\pgfutil@tmpD)"))/2}%
 \pgfmathsetmacro{\pgfutil@tmps}{\pgfutil@tmpA+\pgfutil@tmpB+\pgfutil@tmpC+\pgfutil@tmpD}%
 \pgfmathsetmacro{\pgfutil@tmpA}{\pgfutil@tmpA/\pgfutil@tmps}%
 \pgfmathsetmacro{\pgfutil@tmpB}{\pgfutil@tmpB/\pgfutil@tmps}%
 \pgfmathsetmacro{\pgfutil@tmpC}{\pgfutil@tmpC/\pgfutil@tmps}%
 \pgfmathsetmacro{\pgfutil@tmpD}{\pgfutil@tmpD/\pgfutil@tmps}%
 \pgfmathsetmacro{\pgfutil@tmpI}{TD("\pgfutil@tmpA*\pgfkeysvalueof{/tikz/3d/insphere/A}+\pgfutil@tmpB*\pgfkeysvalueof{/tikz/3d/insphere/B}+\pgfutil@tmpC*\pgfkeysvalueof{/tikz/3d/insphere/C}+\pgfutil@tmpD*\pgfkeysvalueof{/tikz/3d/insphere/D}")}%
 \tikzset{insert path={(\pgfutil@tmpI)}}
},3d/insphere/.cd,A/.initial={(A)},B/.initial={(B)},
C/.initial={(C)},D/.initial={(D)}}%
%
\newif\if@tikz@td@complete@dashes
\@tikz@td@complete@dashesfalse
\tikzset{cheating dash/.code args={on #1 off #2}{%
        %
        \tikz@addoption{%
            \pgfgetpath\pgfutil@tmpc%
            \pgfprocessround{\pgfutil@tmpc}{\pgfutil@tmpc}%
            \pgf@decorate@parsesoftpath{\pgfutil@tmpc}{\pgfutil@tmpc}%
            \pgfmathsetmacro{\pgfutil@tmpa}{\pgf@decorate@totalpathlength-#1}%
            \pgfmathsetmacro{\pgfutil@tmpb}{#1+#2}%
            \pgfmathsetmacro{\pgfutil@tmpd}{max(floor(\pgfutil@tmpa/\pgfutil@tmpb), 1)}%
            \pgfmathsetmacro{\pgfutil@tmpe}{max((\pgfutil@tmpa-\pgfutil@tmpb*\pgfutil@tmpd)/\pgfutil@tmpd+#2,#2)}%
            \pgfsetdash{{#1}{\pgfutil@tmpe}}{0pt}}%
    },cheating dash/.default={on 2pt off 2pt}}%
\tikzset{3d/.cd,%
reset vertex counter/.code={\c@pgf@counta0\relax},
add vertex/.code={\advance\c@pgf@counta by1\relax
\path (#1) coordinate (\the\c@pgf@counta);},
define vertices/.code={\c@pgf@counta0\relax
\tikzset{3d/add vertex/.list={#1}}},%
append vertices/.code={\tikzset{3d/add vertex/.list={#1}}},%
}	
\tikzset{3d/.cd,polyhedron/.cd,
face edges/.style={},
edges have complete dashes/.is if=@tikz@td@complete@dashes,
edges have complete dashes/.default=true,
complete dashes/.code args={on #1 off #2}{\tikzset{%
/tikz/3d/polyhedron/edges have complete dashes=true,
/tikz/3d/polyhedron/face edges/.append style={cheating dash=on #1 off #2}}},
complete dashes/.default={on 2pt off 2pt},
draw face with corners/.code={\begingroup\c@pgf@counta0\relax
\pgfutil@for\pgfutil@tmpa:={#1}\do{%
\pgfmathsetmacro\pgfutil@tmpT{TD("\pgfutil@tmpa")}%
\ifcase\c@pgf@counta 
\pgfmathsetmacro\pgfutil@tmpA{TD("\pgfutil@tmpa")}%
\or
\pgfmathsetmacro\pgfutil@tmpB{TD("\pgfutil@tmpa")}%
\or
\pgfmathsetmacro\pgfutil@tmpC{TD("\pgfutil@tmpa")}%
\fi
\advance\c@pgf@counta by1\relax
\ifnum\c@pgf@counta=1\relax
\edef\pgfutil@tmpl{(\pgfutil@tmpT)}%
\edef\pgfutil@tmplf{(\pgfutil@tmpT)}%
\edef\pgfutil@tmple{(\pgfutil@tmpT)}%
\else
\edef\pgfutil@tmpl{\pgfutil@tmpl -- (\pgfutil@tmpT)}%
\edef\pgfutil@tmple{\pgfutil@tmple\space edge (\pgfutil@tmpT)
(\pgfutil@tmpT)}%
\fi
}%
\ifnum\c@pgf@counta<3\relax
\PackageWarning{3dtools}{A face needs at least three vertices. However, only \the\c@pgf@counta\space vertices were specified.}%
\else
\edef\pgfutil@tmpO{\pgfkeysvalueof{/tikz/3d/polyhedron/O}}%
\pgfmathsetmacro\pgfutil@tmpO{TD("\pgfutil@tmpO")}%
\edef\pgfutil@tmpL{\pgfkeysvalueof{/tikz/3d/polyhedron/L}}%
\pgfmathsetmacro\pgfutil@tmpL{TD("\pgfutil@tmpL")}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)x(\pgfutil@tmpC)-(\pgfutil@tmpA)")}%
\pgfmathsetmacro{\pgfutil@tmpc}{TD("(\pgfutil@tmpA)-(\pgfutil@tmpO)")}%
\pgfmathtruncatemacro{\pgfutil@tmpd}{sign(TD("(\pgfutil@tmpb)o(\pgfutil@tmpc)"))}%
\ifnum\pgfutil@tmpd=-1\relax
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)x(\pgfutil@tmpA)-(\pgfutil@tmpC)")}%
\fi
\pgfmathsetmacro{\pgfutil@tmpe}{screendepth(\pgfutil@tmpb)}%
\pgfmathsetmacro{\pgfutil@tmpf}{sqrt(TD("(\pgfutil@tmpb)o(\pgfutil@tmpb)"))}%
\pgfmathsetmacro{\pgfutil@tmpg}{sqrt(TD("(\pgfutil@tmpL)o(\pgfutil@tmpL)"))}%
\pgfmathsetmacro{\pgfutil@tmph}{TD("(\pgfutil@tmpL)o(\pgfutil@tmpb)")/\pgfutil@tmpf/\pgfutil@tmpg}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{70+30*\pgfutil@tmph}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{\pgfkeysvalueof{/tikz/3d/polyhedron/shading function}(\pgfutil@tmph)}%
\ifdim\pgfutil@tmpe pt<0pt\relax
\begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/polyhedron/back layer}}
\tikzset{3d/polyhedron/before hidden,3d/polyhedron/back}%
\if@tikz@td@complete@dashes
\path[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/back,draw=none] 
	\pgfutil@tmpl -- cycle;
\edef\pgfutil@tmplg{\pgfutil@tmple\space edge \pgfutil@tmplf}%
\draw[3d/polyhedron/back,every edge/.append style={/tikz/3d/polyhedron/face edges}]
	\pgfutil@tmplg;
\else
\draw[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/back] \pgfutil@tmpl -- cycle;
\fi
\tikzset{3d/polyhedron/after hidden}%
\end{pgfonlayer}
\else
\begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/polyhedron/fore layer}}
\tikzset{3d/polyhedron/before visible,3d/polyhedron/fore}%
\if@tikz@td@complete@dashes
\path[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/fore,draw=none]
 \pgfutil@tmpl -- cycle;
\edef\pgfutil@tmplg{\pgfutil@tmple\space edge \pgfutil@tmplf}%
\draw[3d/polyhedron/fore,every edge/.append style={/tikz/3d/polyhedron/face edges}]
	\pgfutil@tmplg;
\else
\draw[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/fore] \pgfutil@tmpl -- cycle;
\fi
\tikzset{3d/polyhedron/after visible}%
\end{pgfonlayer}
\fi
\fi
\endgroup
},
draw open face with corners/.code={\begingroup\c@pgf@counta0\relax
\pgfutil@for\pgfutil@tmpa:={#1}\do{%
\pgfmathsetmacro\pgfutil@tmpT{TD("\pgfutil@tmpa")}%
\ifcase\c@pgf@counta 
\pgfmathsetmacro\pgfutil@tmpA{TD("\pgfutil@tmpa")}%
\or
\pgfmathsetmacro\pgfutil@tmpB{TD("\pgfutil@tmpa")}%
\or
\pgfmathsetmacro\pgfutil@tmpC{TD("\pgfutil@tmpa")}%
\fi
\advance\c@pgf@counta by1\relax
\ifnum\c@pgf@counta=1\relax
\edef\pgfutil@tmpl{(\pgfutil@tmpT)}%
\edef\pgfutil@tmplf{(\pgfutil@tmpT)}%
\edef\pgfutil@tmple{(\pgfutil@tmpT)}%
\else
\edef\pgfutil@tmpl{\pgfutil@tmpl -- (\pgfutil@tmpT)}%
\edef\pgfutil@tmple{\pgfutil@tmple\space edge (\pgfutil@tmpT)
(\pgfutil@tmpT)}%
\fi
}%
\ifnum\c@pgf@counta<3\relax
\PackageWarning{3dtools}{A face needs at least three vertices. However, only \the\c@pgf@counta\space vertices were specified.}%
\else
\edef\pgfutil@tmpO{\pgfkeysvalueof{/tikz/3d/polyhedron/O}}%
\pgfmathsetmacro\pgfutil@tmpO{TD("\pgfutil@tmpO")}%
\edef\pgfutil@tmpL{\pgfkeysvalueof{/tikz/3d/polyhedron/L}}%
\pgfmathsetmacro\pgfutil@tmpL{TD("\pgfutil@tmpL")}%
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)x(\pgfutil@tmpC)-(\pgfutil@tmpA)")}%
\pgfmathsetmacro{\pgfutil@tmpc}{TD("(\pgfutil@tmpA)-(\pgfutil@tmpO)")}%
\pgfmathtruncatemacro{\pgfutil@tmpd}{sign(TD("(\pgfutil@tmpb)o(\pgfutil@tmpc)"))}%
\ifnum\pgfutil@tmpd=-1\relax
\pgfmathsetmacro{\pgfutil@tmpb}{TD("(\pgfutil@tmpB)-(\pgfutil@tmpA)x(\pgfutil@tmpA)-(\pgfutil@tmpC)")}%
\fi
\pgfmathsetmacro{\pgfutil@tmpe}{screendepth(\pgfutil@tmpb)}%
\pgfmathsetmacro{\pgfutil@tmpf}{sqrt(TD("(\pgfutil@tmpb)o(\pgfutil@tmpb)"))}%
\pgfmathsetmacro{\pgfutil@tmpg}{sqrt(TD("(\pgfutil@tmpL)o(\pgfutil@tmpL)"))}%
\pgfmathsetmacro{\pgfutil@tmph}{TD("(\pgfutil@tmpL)o(\pgfutil@tmpb)")/\pgfutil@tmpf/\pgfutil@tmpg}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{70+30*\pgfutil@tmph}%
\pgfmathtruncatemacro{\pgfutil@tmpi}{\pgfkeysvalueof{/tikz/3d/polyhedron/shading function}(\pgfutil@tmph)}%
\ifdim\pgfutil@tmpe pt<0pt\relax
\begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/polyhedron/back layer}}
\tikzset{3d/polyhedron/before hidden,3d/polyhedron/back}%
\if@tikz@td@complete@dashes
\path[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/back,draw=none] 
	\pgfutil@tmpl;
\edef\pgfutil@tmplg{\pgfutil@tmple\space edge \pgfutil@tmplf}%
\draw[3d/polyhedron/back,every edge/.append style={/tikz/3d/polyhedron/face edges}]
	\pgfutil@tmplg;
\else
\draw[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/back] \pgfutil@tmpl ;
\fi
\tikzset{3d/polyhedron/after hidden}%
\end{pgfonlayer}
\else
\begin{pgfonlayer}{\pgfkeysvalueof{/tikz/3d/polyhedron/fore layer}}
\tikzset{3d/polyhedron/before visible,3d/polyhedron/fore}%
\if@tikz@td@complete@dashes
\path[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/fore,draw=none]
 \pgfutil@tmpl ;
\edef\pgfutil@tmplg{\pgfutil@tmple\space edge \pgfutil@tmplf}%
\draw[3d/polyhedron/fore,every edge/.append style={/tikz/3d/polyhedron/face edges}]
	\pgfutil@tmplg;
\else
\draw[fill=tikz@td@face@color!\pgfutil@tmpi!black,3d/polyhedron/fore] \pgfutil@tmpl -- cycle;
\fi
\tikzset{3d/polyhedron/after visible}%
\end{pgfonlayer}
\fi
\fi
\endgroup
},
color/.code={\colorlet{tikz@td@face@color}{#1}},color=yellow,
O/.initial={(0,0,0)},%
L/.initial={(1,1,1)},%
fore/.style={draw,solid},fore layer/.initial=main,
back/.style={draw,dashed,fill opacity=0},back layer/.initial=main,
shading function/.initial={tikztdpolyhedronshade},
/tikz/declare function={tikztdpolyhedronshade(\x)=70+30*\x;},
before visible/.code={},after visible/.code={},
before hidden/.code={},after hidden/.code={},
create face from vertices/.code={\let\pgfutil@tmpa\relax%
\pgfutil@for\pgfutil@tmpb:={#1}\do{%
\ifx\pgfutil@tmpa\relax
\edef\pgfutil@tmpa{{(\pgfkeysvalueof{/tikz/name prefix}\pgfutil@tmpb)}}%
\else
\edef\pgfutil@tmpa{\pgfutil@tmpa,{(\pgfkeysvalueof{/tikz/name prefix}\pgfutil@tmpb)}}%
\fi
}%
\tikzset{3d/polyhedron/draw face with corners/.expanded=\pgfutil@tmpa}%
},%
create faces from vertex list/.style={/tikz/3d/polyhedron/create face from vertices/.list={#1}}%
}%
%
\tikzset{3d/draw named path behind/.code 2 args={%
   %
   \tikzset{3d/current named path=#1,
   	3d/draw named path clipped against/.list={#2},
	3d/draw named path avoiding={#2}}
  },3d/draw named path clipped against/.code={%
  %
  \begin{scope}
   	\clip[use named path/.expanded=#1];
	\draw[3d/hidden,3d/ordered paths/\pgfkeysvalueof{/tikz/3d/current named path}/.try,
		use named path/.expanded=\pgfkeysvalueof{/tikz/3d/current named path}];
  \end{scope}},
  3d/draw named path avoiding/.code={%
  %
  \begin{scope}
   \tikzset{3d/avoid named path/.list={#1}}%
   \draw[3d/visible,3d/ordered paths/\pgfkeysvalueof{/tikz/3d/current named path}/.try,
   	use named path/.expanded=\pgfkeysvalueof{/tikz/3d/current named path}];
  \end{scope}},3d/avoid named path/.code={%
  	\clip[even odd clip,use named path/.expanded=#1,generous outside path];
  },
  3d/current named path/.initial={},
  3d/draw ordered paths/.code={%
  \tikzset{3d/temporary list 1/.initial={#1},
  	3d/draw ordered path/.list={#1}}%
  },3d/draw ordered path/.code={%
  %
  \expanded{\noexpand\pgfutil@in@{,}{\pgfkeysvalueof{/tikz/3d/temporary list 1}}}%
  \tikzset{3d/temporary list 1/.remove item={#1}}
  \ifpgfutil@in@%
	\tikzset{3d/draw named path behind/.expanded={#1}{\pgfkeysvalueof{/tikz/3d/temporary list 1}}} 
  \else
   \begin{scope}
	\draw[3d/visible,3d/ordered paths/#1/.try,
	use named path/.expanded=#1];
   \end{scope}	
  \fi  
  },3d/ordered paths/.unknown/.code={}}
%
\tikzset{pics/ycylinder/.style={code={%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\tikzset{3d/.cd,#1}%
%
\pgfmathsetmacro{\tikz@td@vmin}{-atan2(sin(\pgfkeysvalueof{/tikz/3d/phi})*sin(\pgfkeysvalueof{/tikz/3d/theta}),cos(\pgfkeysvalueof{/tikz/3d/theta}))}%
\pgfmathsetmacro{\tikz@td@vmax}{\tikz@td@vmin+180}%
\path[3d/cylinder/mantle]
  let \p1=($(0,1,0)-(0,0,0)$),\n1={atan2(\y1,\x1)+180} in
  [shading angle=\n1]
  plot[variable=\tikz@td@t,domain=\tikz@td@vmin:\tikz@td@vmax,smooth]
    ({\pgfkeysvalueof{/tikz/3d/r}*cos(\tikz@td@t)},0,{\pgfkeysvalueof{/tikz/3d/r}*sin(\tikz@td@t)})
    -- 
    plot[variable=\tikz@td@t,domain=\tikz@td@vmax:\tikz@td@vmin,smooth]
    ({\pgfkeysvalueof{/tikz/3d/r}*cos(\tikz@td@t)},\pgfkeysvalueof{/tikz/3d/h},{\pgfkeysvalueof{/tikz/3d/r}*sin(\tikz@td@t)})
    --cycle;
\pgfmathtruncatemacro{\tikz@td@i}{sign(cos(\pgfkeysvalueof{/tikz/3d/phi}))}%
\ifnum\tikz@td@i=-1\relax
\pgfmathtruncatemacro{\tikz@td@i}{sign(cos(\pgfkeysvalueof{/tikz/3d/phi}))}%
    \path[3d/cylinder/top] plot[variable=\tikz@td@t,domain=0:360,smooth cycle]
    ({\pgfkeysvalueof{/tikz/3d/r}*cos(\tikz@td@t)},\pgfkeysvalueof{/tikz/3d/h},{\pgfkeysvalueof{/tikz/3d/r}*sin(\tikz@td@t)}) ;
\fi
\ifnum\tikz@td@i=1\relax
    \path[3d/cylinder/top] plot[variable=\tikz@td@t,domain=0:360,smooth cycle]
    ({\pgfkeysvalueof{/tikz/3d/r}*cos(\tikz@td@t)},0,{\pgfkeysvalueof{/tikz/3d/r}*sin(\tikz@td@t)}) ;
\fi
}},pics/cylinder/.style={code={%
%
\tikzset{3d/.cd,#1}%
\pgfmathsetmacro{\tikz@td@v}{TD("\pgfkeysvalueof{/tikz/3d/cylinder/axis}x(nscreenx,nscreeny,nscreenz)")}%
\pgfmathtruncatemacro{\tikz@td@i}{abs(TD("(\tikz@td@v)o(\tikz@td@v)"))>0.01?1:0}%
\ifnum\tikz@td@i=0\relax 
  \path[3d/cylinder/top] circle[radius=\pgfkeysvalueof{/tikz/3d/r}];
\else 
  \pgfmathsetmacro{\tikz@td@ex}{TDunit("\pgfkeysvalueof{/tikz/3d/cylinder/axis}x(nscreenx,nscreeny,nscreenz)")}%
  \pgfmathsetmacro{\tikz@td@ey}{TDunit("(\tikz@td@ex)x\pgfkeysvalueof{/tikz/3d/cylinder/axis}")}%
  \pgfmathtruncatemacro{\tikz@td@i}{TD("\pgfkeysvalueof{/tikz/3d/cylinder/axis}o(nscreenx,nscreeny,nscreenz)")>0?1:0}%
  \ifnum\tikz@td@i=1\relax 
    \pgfmathsetmacro{\tikz@td@ey}{TD("-1*(\tikz@td@ey)")}%
  \else
    %
  \fi
  \pgfmathsetmacro{\tikz@td@ez}{TDunit("\pgfkeysvalueof{/tikz/3d/cylinder/axis}")}%
  \expanded{\noexpand\path[overlay,
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ex}=(\tikz@td@ex)},
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ey}=(\tikz@td@ey)},
	3d coordinate={\pgfkeysvalueof{/tikz/3d/aux keys/ez}=(\tikz@td@ez)}];}%
  \pgfmathtruncatemacro{\tikz@td@i}{TD("\pgfkeysvalueof{/tikz/3d/cylinder/axis}o(nscreenx,nscreeny,nscreenz)")>0?1:0}%
  \begin{scope}[x/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ex}},
    y/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ey}},
    z/.expanded={\pgfkeysvalueof{/tikz/3d/aux keys/ez}}]       
    \ifnum\tikz@td@i=1\relax 
      \draw[3d/hidden] (\pgfkeysvalueof{/tikz/3d/r},0,0) arc[start angle=0,end angle=180,radius=\pgfkeysvalueof{/tikz/3d/r}];
    \else 
      \draw[3d/hidden] (\pgfkeysvalueof{/tikz/3d/r},0,\pgfkeysvalueof{/tikz/3d/h}) arc[start angle=0,end angle=180,radius=\pgfkeysvalueof{/tikz/3d/r}];
    \fi
    \path[3d/cylinder/mantle]
      let \p1=($(0,1,0)-(0,0,0)$),\n1={atan2(\y1,\x1)+180} in
      [shading angle=\n1]
      (\pgfkeysvalueof{/tikz/3d/r},0,0) arc[start angle=0,end angle=-180,radius=\pgfkeysvalueof{/tikz/3d/r}]
        -- 
      ({-1*(\pgfkeysvalueof{/tikz/3d/r})},0,\pgfkeysvalueof{/tikz/3d/h}) arc[start angle=-180,end angle=0,radius=\pgfkeysvalueof{/tikz/3d/r}]
      -- cycle;
    \ifnum\tikz@td@i=1\relax 
      \path[3d/cylinder/top] (0,0,\pgfkeysvalueof{/tikz/3d/h}) circle[radius=\pgfkeysvalueof{/tikz/3d/r}];
    \else 
      \path[3d/cylinder/top] (0,0,0) circle[radius=\pgfkeysvalueof{/tikz/3d/r}];
    \fi
  \end{scope}  
\fi
}},%
3d/.cd,cylinder/.cd,
mantle/.style={draw},top/.style={draw}}
\tikzset{3d/.cd,visible/.style={draw,solid},
	hidden/.style={draw,very thin,cheating dash},
	r/.initial=1,h/.initial=1,R/.initial=2,
  cylinder/axis/.initial={(0,0,1)}}
%
%
%
%
\newcounter{tikz@td@recorded@point}
\pgfmathdeclarefunction{tikztdindexoflastcoordinate}{0}{%
\edef\pgfmathresult{\number\value{tikz@td@recorded@point}}%
}%

\tikzset{stored path/.cd,coordinate prefix/.initial={stored-},
	reset coordinate index/.code={\setcounter{tikz@td@recorded@point}{0}},
	restore path/.style={insert path/.expanded={\csname tikz@td@recorded@path@f@#1\endcsname}},%
	restore reversed path/.style={insert path/.expanded={\csname tikz@td@recorded@path@r@#1\endcsname}},%
	append path/.style={insert path/.expanded={-- \csname tikz@td@recorded@path@f@#1\endcsname}},%
	append reversed path/.style={insert path/.expanded={-- \csname tikz@td@recorded@path@r@#1\endcsname}},%
	first coordinate of/.style={insert path/.expanded={(\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-0)}},%
	last coordinate of/.style={insert path/.expanded={(\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-\the\numexpr\value{tikz@td@recorded@point})}},%
	coordinate with index/.style args={#1 of #2}{insert path/.expanded={(\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#2-#1)}},%
/tikz/extend stored path/.style={%
	%
    decorate,decoration={show path construction,
    moveto code={\def\tikz@td@prefix{\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-}%
	\path (\tikzinputsegmentfirst) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point});
    \ifnum\value{tikz@td@recorded@point}=0
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	\else
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{%
	 	\csname tikz@td@recorded@path@f@#1\endcsname
		(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}) 
		\csname tikz@td@recorded@path@r@#1\endcsname}%
	\fi
	\stepcounter{tikz@td@recorded@point}%
    },
    lineto code={\def\tikz@td@prefix{\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-}%
	\path (\tikzinputsegmentfirst) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		 (\tikzinputsegmentlast) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1);
    \ifnum\value{tikz@td@recorded@point}=0
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	\else
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{%
	 	\csname tikz@td@recorded@path@f@#1\endcsname
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1) --
		\csname tikz@td@recorded@path@r@#1\endcsname}%
	\fi
	\stepcounter{tikz@td@recorded@point}%
    },
    curveto code={\def\tikz@td@prefix{\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-}%
      \path (\tikzinputsegmentfirst)
	    coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
        (\tikzinputsegmentsupporta) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		(\tikzinputsegmentsupportb)
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
        (\tikzinputsegmentlast)
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3);
    \ifnum\value{tikz@td@recorded@point}=0
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		.. controls (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		and (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
		.. (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3)
		.. controls (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
		and (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		.. (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	\else
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{%
	 	\csname tikz@td@recorded@path@f@#1\endcsname
		.. controls (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		and (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
		.. (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+3)
		.. controls (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+2)
		and (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1) ..
		\csname tikz@td@recorded@path@r@#1\endcsname}%
	\fi
	\stepcounter{tikz@td@recorded@point}%
	\stepcounter{tikz@td@recorded@point}%
	\stepcounter{tikz@td@recorded@point}%
    },
    closepath code={\def\tikz@td@prefix{\pgfkeysvalueof{/tikz/stored path/coordinate prefix}#1-}%
	\path (\tikzinputsegmentfirst) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		 (\tikzinputsegmentlast) 
		coordinate (\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1);
    \ifnum\value{tikz@td@recorded@point}=0
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point})}%
	\else
	 \expandafter\xdef\csname tikz@td@recorded@path@f@#1\endcsname{%
	 	\csname tikz@td@recorded@path@f@#1\endcsname
		--(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1)}%
	 \expandafter\xdef\csname tikz@td@recorded@path@r@#1\endcsname{%
	 	(\tikz@td@prefix\the\numexpr\value{tikz@td@recorded@point}+1) --
		\csname tikz@td@recorded@path@r@#1\endcsname}%
	\fi
	  } }},
/tikz/store path/.style={%
	  /tikz/stored path/reset coordinate index,%
	  /tikz/extend stored path=#1}
	  }
%
\def\tikz@td@bbox@store@aux#1#2{%
	\immediate\write\@mainaux{\string\expandafter\xdef\noexpand\csname pgfk@/tikz/3d/bbox/stored/#1\string\endcsname{#2}}%
	\expandafter\xdef\csname pgfk@/tikz/3d/bbox/stored/#1\endcsname{#2}}%
\def\tikz@td@bbox@@get@min@from@aux#1#2{%
	\ifcsname pgfk@/tikz/3d/bbox/stored/#1min\endcsname
	\edef#2{\csname pgfk@/tikz/3d/bbox/stored/#1min\endcsname}%
	\else
	\edef#2{16383.99999pt}%
	\expandafter\edef\csname pgfk@/tikz/3d/bbox/stored/#1min\endcsname{16383.99999pt}%
	\fi}
\def\tikz@td@bbox@@get@max@from@aux#1#2{%
	\ifcsname pgfk@/tikz/3d/bbox/stored/#1max\endcsname
	\edef#2{\csname pgfk@/tikz/3d/bbox/stored/#1max\endcsname}%
	\else
	\edef#2{-16383.99999pt}%
	\expandafter\edef\csname pgfk@/tikz/3d/bbox/stored/#1max\endcsname{-16383.99999pt}%
	\fi}
\tikzset{same bounding box/.style={%
execute at end picture={%
\tikz@td@bbox@@get@min@from@aux{#1x}\pgfutil@tmpa%
\tikz@td@bbox@@get@min@from@aux{#1y}\pgfutil@tmpb%
\tikz@td@bbox@@get@max@from@aux{#1x}\pgfutil@tmpc%
\tikz@td@bbox@@get@max@from@aux{#1y}\pgfutil@tmpd%
%
\pgfmathsetmacro\pgfutil@tmpa{min(\pgfutil@tmpa,\pgf@picminx,\pgfkeysvalueof{/tikz/3d/bbox/stored/#1xmin})}%
\pgfmathsetmacro\pgfutil@tmpb{min(\pgfutil@tmpb,\pgf@picminy,\pgfkeysvalueof{/tikz/3d/bbox/stored/#1ymin})}%
\pgfmathsetmacro\pgfutil@tmpc{max(\pgfutil@tmpc,\pgf@picmaxx,\pgfkeysvalueof{/tikz/3d/bbox/stored/#1xmax})}%
\pgfmathsetmacro\pgfutil@tmpd{max(\pgfutil@tmpd,\pgf@picmaxy,\pgfkeysvalueof{/tikz/3d/bbox/stored/#1ymax})}%
%
\tikz@td@bbox@store@aux{#1xmin}{\pgfutil@tmpa}%
\tikz@td@bbox@store@aux{#1ymin}{\pgfutil@tmpb}%
\tikz@td@bbox@store@aux{#1xmax}{\pgfutil@tmpc}%
\tikz@td@bbox@store@aux{#1ymax}{\pgfutil@tmpd}%
\ifdim\pgfutil@tmpa pt<16383.99999pt\relax
\path (\pgfutil@tmpa pt,\pgfutil@tmpb pt) (\pgfutil@tmpc pt,\pgfutil@tmpd pt);
\fi
}},same bounding box/.default=A} 	  
%
\newif\if@pgf@list@first@item
\pgfkeys{/handlers/.add item/.code=\pgfkeys{\pgfkeyscurrentpath/.append={,#1}},
/handlers/.remove item/.code={%
\edef\pgfutil@tmpa{\pgfkeysvalueof{\pgfkeyscurrentpath}}%
\edef\pgfutil@tmpb{#1}%
\edef\pgfutil@tmpc{\noexpand\@removeelement{\pgfutil@tmpb}{\pgfutil@tmpa}{\noexpand\pgfutil@tmpa}}%
\pgfutil@tmpc
\pgfkeyssetvalue{\pgfkeyscurrentpath}{\pgfutil@tmpa}},%
/handlers/.count/.code={\begingroup%
\edef\pgfutil@tmpl{\pgfkeysvalueof{\pgfkeyscurrentpath}}%
\c@pgf@counta0\relax
\pgfkeys{/list management/step count/.list/.expanded={\pgfutil@tmpl}}%
\edef#1{\the\c@pgf@counta}%
\pgfmathsmuggle#1\endgroup},%
/handlers/.print list/.code={\begingroup%
\@pgf@list@first@itemtrue
\edef\pgfutil@tmpl{\pgfkeysvalueof{\pgfkeyscurrentpath}}%
\pgfkeys{/list management/print item in list/.list/.expanded={\pgfutil@tmpl}}%
\endgroup},
/handlers/.is array/.code={\pgfkeysifdefined{\pgfkeyscurrentpath}{%
\typeout{The key `\pgfkeyscurrentpath` is already in use, and won't get overwritten.}}{%
\pgfkeysifdefined{\pgfkeyscurrentpath/dim}{%
\typeout{The key `\pgfkeyscurrentpath` is already in use, and won't get overwritten.}}{%
\c@pgf@counta=0\relax
\pgfkeyssetevalue{/list management/current array}{\pgfkeyscurrentpath}%
\pgfkeys{/list management/store array entry/.list/.expanded={#1}}%
\pgfkeys{\pgfkeysvalueof{/list management/current array}/dim/.initial=\the\c@pgf@counta}%
\pgfkeys{\pgfkeysvalueof{/list management/current array}/content/.initial={#1}}%
}}},
/handlers/.sort numeric list/.code 2 args={\begingroup%
\edef\pgfutil@tmpl{\pgfkeysvalueof{\pgfkeyscurrentpath}}%
\edef\pgfutil@tmpa{0}%
\pgfutil@for\pgfutil@tmpb:={\pgfutil@tmpl}\do{%
\edef\pgfutil@tmpa{\the\numexpr\pgfutil@tmpa+1}%
\ifcase\pgfutil@tmpa
\or
\or
\edef\pgfutil@tmph{2}%
\else
\edef\pgfutil@tmph{\pgfutil@tmph,\pgfutil@tmpa}%
\fi
\pgfkeys{/list management/sort map=\pgfutil@tmpb}%
\expandafter\edef\csname pgfutil@tmpd@\pgfutil@tmpa\endcsname{\pgfmathresult}%
\expandafter\edef\csname pgfutil@tmpf@\pgfutil@tmpa\endcsname{\pgfutil@tmpa}%
}%
\edef\pgfutil@tmps{\pgfkeysvalueof{/list management/sort comparison}}%
\pgfutil@loop
\edef\pgfutil@tmpi{1}%
\pgfutil@for\pgfutil@tmpb:={\pgfutil@tmph}\do{%
\edef\pgfutil@tmpx{\@nameuse{pgfutil@tmpd@\pgfutil@tmpb}}%
\edef\pgfutil@tmpc{\the\numexpr\pgfutil@tmpb-1}%
\edef\pgfutil@tmpy{\@nameuse{pgfutil@tmpd@\pgfutil@tmpc}}%
\edef\pgfutil@tmpr{(\pgfutil@tmpx\pgfutil@tmps\pgfutil@tmpy?1:0)}%
\pgfmathtruncatemacro\pgfutil@tmpj{\pgfutil@tmpr}%
\ifnum\pgfutil@tmpj=0\relax
\edef\pgfutil@tmpi{0}%
\edef\pgfutil@tmpu{\@nameuse{pgfutil@tmpf@\pgfutil@tmpb}}%
\edef\pgfutil@tmpv{\@nameuse{pgfutil@tmpf@\pgfutil@tmpc}}%
%
\expandafter\edef\csname pgfutil@tmpd@\pgfutil@tmpb\endcsname{\pgfutil@tmpy}%
\expandafter\edef\csname pgfutil@tmpd@\pgfutil@tmpc\endcsname{\pgfutil@tmpx}%
\expandafter\edef\csname pgfutil@tmpf@\pgfutil@tmpb\endcsname{\pgfutil@tmpv}%
\expandafter\edef\csname pgfutil@tmpf@\pgfutil@tmpc\endcsname{\pgfutil@tmpu}%
\fi
}%
\ifnum\pgfutil@tmpi=0\relax
\pgfutil@repeat
\edef\pgfutil@tmpa{\@nameuse{pgfutil@tmpf@1}}%
\edef\pgfutil@tmpc{\@nameuse{pgfutil@tmpd@1}}%
\pgfutil@for\pgfutil@tmpb:={\pgfutil@tmph}\do{%
\edef\pgfutil@tmpa{\pgfutil@tmpa,\@nameuse{pgfutil@tmpf@\pgfutil@tmpb}}%
\edef\pgfutil@tmpc{\pgfutil@tmpc,\@nameuse{pgfutil@tmpd@\pgfutil@tmpb}}}%
\edef\pgfutil@tmpb{\noexpand\edef\noexpand#1{\pgfutil@tmpc}\noexpand\edef\noexpand#2{\pgfutil@tmpa}}%
\pgfmathsmuggle\pgfutil@tmpb\endgroup\pgfutil@tmpb},
/list management/.cd,print item/.code={#1},
print item in list/.code={%
\if@pgf@list@first@item
 \pgfkeys{/list management/print item={#1}}%
 \@pgf@list@first@itemfalse
\else
 \pgfkeys{/list management/print item={%
  \pgfkeysvalueof{/list management/list separator}#1}}%
\fi},
list separator/.initial={,\space},
step count/.code={\advance\c@pgf@counta by1\relax},
sort comparison/.initial={>=},
sort map/.code={\pgfmathparse{#1}},
current array/.initial={},
store array entry/.code={\advance\c@pgf@counta by1\relax
\pgfkeyssetevalue{\pgfkeysvalueof{/list management/current array}/\the\c@pgf@counta}{#1}}
}%
%
\newif\ifcoil@closed%
\pgfkeys{%
/pgf/decoration/.cd,%
3d coil color/.initial=black,%
3d coil width/.initial=0.4pt,%
3d coil dist/.initial=0.6pt,%
3d coil opacity/.initial=1,%
3d coil closed/.code=\coil@closedtrue%
}%
%
%
%
%
%
%
%
%
%
%
%
\def\pgfpoint@onthreedcoil#1#2#3{%
  \pgf@x=#1\pgfdecorationsegmentamplitude%
  \pgf@x=\pgfdecorationsegmentaspect\pgf@x%
  \pgf@y=#2\pgfdecorationsegmentamplitude%
  \pgf@xa=0.083333333333\pgfdecorationsegmentlength%
  \advance\pgf@x by#3\pgf@xa%
  \advance\pgf@x by-\generaloffset pt%
}%
%
%
%
\pgfdeclaredecoration{3d complete coil}{initial}%
{ %
    \state{initial}[width=0.5*\pgfdecorationsegmentlength,%
    next state=coil, persistent precomputation={%
    \pgfmathsetmacro\matchinglength{\pgfdecoratedinputsegmentlength / int(\pgfdecoratedinputsegmentlength/\pgfdecorationsegmentlength)}%
    \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}%
    %
    \pgfmathsetmacro{\generaloffset}{\pgfdecorationsegmentlength}%
    \pgfmathsetmacro{\initialoffset}{1.5*\pgfdecorationsegmentlength}%
    \pgfmathsetmacro{\auxoffset}{2.5*\pgfdecorationsegmentlength}%
  }]    { %
    %
    %
	\edef\TDCoilColor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
	\edef\TDCoilOpacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
	\edef\TDCoilWidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}}%
	\edef\TDCoilDist{\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}}     %
    \ifcoil@closed%
     \begingroup%
      \def\generaloffset{\auxoffset}%
      \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
      \pgfpathcurveto%
      {\pgfpoint@onthreedcoil{1.555}{ 1    }{16}}%
      {\pgfpoint@onthreedcoil{2    }{ 0.555}{17}}%
      {\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
      \pgfcoordinate{TD@coilast}{\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
      \pgfcoordinate{TD@coilfirst}{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
      \pgfusepath{stroke} %
      \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \endgroup%
    \fi%
    \begingroup %
    \def\generaloffset{\initialoffset}%
    \ifcoil@closed%
     \pgfpathmoveto{\pgfpointanchor{TD@coilast}{center}}%
    \else%
     \pgfpathmoveto{\pgfpointorigin}%
    \fi%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{2    }{-0.555}{7}}%
    {\pgfpoint@onthreedcoil{1.555}{-1    }{8}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke} %
    %
    %
    %
    \pgfsetstrokeopacity{1}%
    \pgfsetstrokecolor{white}%
    \pgfsetfillcolor{white}%
    \pgfsetlinewidth{1.5*\pgfkeysvalueof{/pgf/decoration/3d coil width}+1.5*\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
    {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke,fill} %
    %
    %
    %
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
    %
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
    {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke,fill} %
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{1.555}{ 1    }{16}}%
    {\pgfpoint@onthreedcoil{2    }{ 0.555}{17}}%
    {\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
    \pgfcoordinate{TD@coilast}{\pgfpoint@onthreedcoil{2    }{ 0    }{18}} %
    \pgfusepath{stroke}     %
    \endgroup%
  }%
  \state{coil}[switch if less than=%
    1.9*\pgfdecorationsegmentlength  to last,%
               width=+\pgfdecorationsegmentlength]%
    { %
    %
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfpathmoveto{\pgfpointanchor{TD@coilast}{center}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{2    }{-0.555}{7}}%
    {\pgfpoint@onthreedcoil{1.555}{-1    }{8}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke} %
    %
    %
    %
    \pgfsetstrokeopacity{1}%
    \pgfsetstrokecolor{white}%
    \pgfsetfillcolor{white}%
    \pgfsetlinewidth{1.5*\pgfkeysvalueof{/pgf/decoration/3d coil width}+1.5*\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
    {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke,fill} %
    %
    %
    %
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
    %
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
    {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
    {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
    {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
    {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke,fill} %
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{1.555}{ 1    }{16}}%
    {\pgfpoint@onthreedcoil{2    }{ 0.555}{17}}%
    {\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
    \pgfusepath{stroke} %
    \pgfcoordinate{TD@coilast}{\pgfpoint@onthreedcoil{2    }{ 0    }{18}} %
  }%
  \state{last}[next state=final]%
    { %
    %
    \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
    \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
    \pgfpathmoveto{\pgfpointanchor{TD@coilast}{center}}%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
    \pgfpathcurveto%
    {\pgfpoint@onthreedcoil{2    }{-0.555}{7}}%
    {\pgfpoint@onthreedcoil{1.555}{-1    }{8}}%
    {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
    \pgfusepath{stroke} %
    %
    %
    %
    \ifcoil@closed %
     %
     %
     %
     \pgfsetstrokeopacity{1}%
     \pgfsetstrokecolor{white}%
     \pgfsetfillcolor{white}%
     \pgfsetlinewidth{1.5*\pgfkeysvalueof{/pgf/decoration/3d coil width}+1.5*\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     %
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
     {\pgfpointanchor{TD@coilfirst}{center}}%
     %
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfusepath{stroke,fill} %
     \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{3}}%
     \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
     %
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
     {\pgfpointanchor{TD@coilfirst}{center}}%
     %
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfusepath{stroke,fill} %
    \else%
     %
     %
     %
     \pgfsetstrokeopacity{1}%
     \pgfsetstrokecolor{white}%
     \pgfsetfillcolor{white}%
     \pgfsetlinewidth{1.5*\pgfkeysvalueof{/pgf/decoration/3d coil width}+1.5*\pgfkeysvalueof{/pgf/decoration/3d coil dist}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1}{1}{3}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1}{-1}{9}}%
     %
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
     {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
     %
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfusepath{stroke,fill} %
     \pgfsetstrokecolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \pgfsetfillcolor{\pgfkeysvalueof{/pgf/decoration/3d coil color}}%
     \pgfsetstrokeopacity{\pgfkeysvalueof{/pgf/decoration/3d coil opacity}}%
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1}{1}{3}}%
     \pgfsetlinewidth{\pgfkeysvalueof{/pgf/decoration/3d coil width}} %
     %
     \pgfpathmoveto{\pgfpoint@onthreedcoil{1}{-1}{9}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{11.25}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{12.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{13.25}}%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14.25}}%
     {\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
     %
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0.445}{ 1    }{14}}%
     {\pgfpoint@onthreedcoil{0    }{ 0.555}{12.75}}%
     {\pgfpoint@onthreedcoil{0    }{ 0    }{11.5}}%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{0    }{-0.555}{10.75}}%
     {\pgfpoint@onthreedcoil{0.445}{-1    }{10}}%
     {\pgfpoint@onthreedcoil{1    }{-1    }{9}}%
     \pgfusepath{stroke,fill} %
    \fi%
    \pgfpathmoveto{\pgfpoint@onthreedcoil{1    }{ 1    }{15}}%
    \ifcoil@closed %
    \else%
     \pgfpathcurveto%
     {\pgfpoint@onthreedcoil{1.555}{ 1    }{16}}%
     {\pgfpoint@onthreedcoil{2    }{ 0.555}{17}}%
     {\pgfpoint@onthreedcoil{2    }{ 0    }{18}}%
    \fi%
    \pgfusepath{stroke} %
    %
  }%
  \state{final}%
  {%
    \pgfpathmoveto{\pgfpointdecoratedpathlast}%
	\pgfutil@namelet{\string\color@pgfstrokecolor}{pgf@strokecolor@global}%
    %
  }%
}%
%
%
\newcounter{tikz@td@cone@shading}
%
\tikzset{3d/cone/shading/.cd,x/.initial=0,y/.initial=0,alpha/.initial=0,
brightness/.initial=0.5,
create shading/.code={%
\stepcounter{tikz@td@cone@shading}%
\tikzset{3d/cone/shading/.cd,#1}%
\pgfdeclarefunctionalshading{simple cone \number\value{tikz@td@cone@shading}}{\pgfpoint{-25bp}{-25bp}}{\pgfpoint{25bp}{25bp}}{}{
    %
	\pgfkeysvalueof{/tikz/3d/cone/shading/y} -1 mul add %
	exch %
	\pgfkeysvalueof{/tikz/3d/cone/shading/x} -1 mul add %
	exch %
    atan   %
	\pgfkeysvalueof{/tikz/3d/cone/shading/alpha} add %
    sin         %
	1 add       %
    \pgfkeysvalueof{/tikz/3d/cone/shading/brightness} mul     %
    dup mul     %
	2 mul
	dup dup		%
}}}
\tikzset{3d/cone shading/.style={3d/cone/shading/create shading={#1},
 shading=simple cone \number\value{tikz@td@cone@shading}}}
\makeatother
\endinput

